Generating High Fidelity Data from Low-density Regions using Diffusion Models

Our work focuses on addressing sample deficiency from low-density regions of data manifold in common image datasets. We leverage diffusion process based generative models to synthesize novel images from low-density regions. We observe that uniform sampling from diffusion models predominantly samples from high-density regions of the data manifold. Therefore, we modify the sampling process to guide it towards low-density regions while simultaneously maintaining the fidelity of synthetic data. We rigorously demonstrate that our process successfully generates novel high fidelity samples from low-density regions. We further examine generated samples and show that the model does not memorize low-density data and indeed learns to generate novel samples from low-density regions.

==> Diverse sampling from generative models [CVPR 22]/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Diverse sampling from generative models [CVPR 22]/sections/applications.tex <==
% Two ways to compare results. 
% 1. Uniforms vs synthetic ours: How much does distribution coverage benefits us. May be not too much as we don't have much samples in high density regions, which real data expects. May be see if we stable more on robustness. 
% Plot the final hardness score of both ours and baseline to give some context there.
% 2. 



==> Diverse sampling from generative models [CVPR 22]/sections/introduction.tex <==
Most common image datasets have a long-tailed distribution of sample density\footnote{We refer to the long-tail~\wrt sample density for each class. It is different from the long-tailed distribution over classes~\cite{liu2019ImageNetLongTail},~\ie, when some classes are heavily underrepresented than others.}, where the majority of samples lie in high-density neighborhoods of the data manifold. Samples from low-density regions often comprise novel attributes (Figure~\ref{fig:teaser}a) and have higher entropy than high-density samples~\cite{agarwal2020VOG}. However, due to their lower likelihood, curating even a small amount of such samples requires a dedicated effort~\cite{hendrycks2021naturalAdv}. 

% Thus real world samples from low-density regions, which have higher entropy and often contain novel attributes (Figure~\ref{fig:teaser}a), are hard to collect. Even collecting a very small amount of such real low-density samples often requires a dedicated effort~\cite{hendrycks2021naturalAdv}. 
% Another interpretation of it is that majority of samples (high-density) share common class attributes, a very small nu
% mber of samples (low-density) include a unique variation of class attributes (fig. 1a).

Our goal is to leverage generative models to generate synthetic images from low-density neighborhoods. A natural requirement for this task is that the model should generalize to low-density regions. While generative adversarial networks (GANs) excel at generating high-fidelity samples, they have poor coverage, thus struggle to generate high-fidelity samples from low-density regions~\cite{brock2018bigGandeep} (Figure~\ref{fig:teaser}b). In contrast, autoregressive models have a high coverage but fail to generate high fidelity images~\cite{child2019sparseTransformer}.  We use diffusion-based models due to their ability to achieve high fidelity and high coverage of the distribution, simultaneously~\cite{ho2020denoisingdiffusion, nichol2021improvedDdpm}.

% We argue that synthetic data can address the deficiency of samples from low-density regions in natural datasets. Our work leverage diffusion-based probabilistic models (DDPM)~\cite{ho2020denoisingdiffusion} to generate novel synthetic images from the low-density regions of the data manifold.

% Data manifold has both high density and low density components. Real-dataset itself is log-tailed, i.e., samples unique attributes. e.g., color number of object variations. Our work focuses on generating synthetic data from low-density regions. Real data is long-tailed, large number of samples in high-density. If we train a generative model on such long-tailed distribution, how do we generate novel low-density samples.  

% Modelling/Interpolating low-density regions has always been a challenge for generative models. GANs achieve high fidelity but fails to cover modes. Transformers based model have coverage (do they) but doesn't achieve high fidelity samples. We focus on the recent success of energy based models, in particular, diffusion based generative models, which achieve high mode coverage while high fidelity.

% where $\mu_{\theta}(x_t, t)$ and $\Sigma_{\theta}(x_t, t)$ are the mean the standard deviation generated by the neural network parameterized by $\theta$. $z$ is sampled from from $\gN(0, 1)$. Gradients from network $f_a$ guided the sampling process towards low-density regions while $f_b$ network forces the process to stay close to the data distribution. $\nabla^*$ refers to normalized gradients. We normalize gradients to disentangle the choice of hyperparameters $\alpha$ and $\beta$ from the diffusion process timesteps ($t$). 

% Diffusion models are trained to maximize the variational lower bounds on the likelihood of the training data. We commonly use annealed Langevin dynamics to sample data from them. We add additional terms to guide it towards low-density regions. 

In training diffusion models, the goal is to approximate data distribution, which is often long-tailed. Diffusion models excel at this task, as we observe that the density distribution of uniformly sampled instances from the diffusion model is very similar to real data. 

Thus uniform sampling from these models leads to an imitation of real data density distribution, i.e., a long-tailed density distribution, where it generates samples from high-density regions with a much higher probability than from low-density regions (figure~\ref{fig:teaser}c). 
% However, when closely approximating real data distribution, baseline sampling also leads to a long-tailed density distribution, i.e., it generates samples from high-density regions with a much higher probability than from low-density regions (figure~\ref{fig:teaser}c). 
To alleviate this issue, we first modify the sampling process to include an additional guidance signal to steer it towards low-density neighborhoods. However, at higher magnitudes of this signal, the generative process is steered off the manifold, thus generating low fidelity samples. We circumvent this challenge by including a second guidance signal which incentives diffusion models to generate samples that are close to the real data manifold.

% We argue that it is necessary to include the additional guidance term (based on network $f_b$) to stay close to the data manifold. In absence of it, larger values of $\alpha$ will steer the sampling process away from the data manifold, thus generating low fidelity images. By controlling the hyperparameter ($\alpha$, $\beta$), our framework enables the generation of high-fidelity synthetic images from low-density regions of data manifold (fig. 2). We also provide a quantitative comparison of our approach with baseline, which demonstrates that our approach outperforms baselines across multiple metrics for data density, such as Gaussian likelihoods, k-nearest neighbors, probabilistic PCA, etc~\cite{devries2020instanceSelection}. 

% These models are trained by maximizing a lower-bound on likelihood. In sampling, it imitates training data and achieve a long-tailed distribution. How do we control the sampling process to guide it towards sampling region, while maintaining the fidelity of samples. 

% We control an addition term to generate low likelihood samples. However, the model can easily cheat by generating non-realistic images, we further add another term to force it stay close to data distribution. 
% Success: We first visually analyze the impact of both term. Next we compare the density of samples generated form our approach with baselines, showing that our approach can provide a very effective control.

Since a very limited number of training samples are available from low-density regions, it is natural to ask whether diffusion models are generalizing in the low-density regions or simply memorizing the training data. After all, recent works have uncovered such memorization in language-based generative models~\cite{carlini2021LmMemorization, carlini2019secretSharer}. We conduct an extensive analysis to justify that diffusion models do not show signs of memorizing training samples from low-density neighborhoods and indeed learn to interpolate in these regions. We make the following key contributions.
% We also delve deeper into multiple other aspects of our framework such as integration with fast sampling procedures, connection to adversarial examples in the sampling process, and class-wise interpolation ability.\\

\begin{itemize}[noitemsep,topsep=5pt,parsep=5pt,partopsep=0pt]
    \item We propose an improved sampling process for diffusion models that can generate samples from low-density neighborhoods of the training data manifold. 
    \item We validate the success of our approach using three different metrics for neighborhood density and provide extensive comparisons with the baseline sampling process in diffusion models. 
    \item We show that our sampling process successfully generates novel samples, which aren't simply memorized training samples, from low-density regions. This observation from our sampling process also uncover that despite a limited number of training images available from low-density regions, diffusion models successfully generalize in low-density regions. 
\end{itemize}

\section{Related work}
Diffusion-based probabilistic models~\cite{ho2020denoisingdiffusion, nichol2021improvedDdpm, dhariwal2021diffBeatGANs} and its closely related variants~\cite{song2019ScoreEstimateGrad, song2020ImprovedTechScore} are likelihood-based models that learns data distribution by learning the reverse process of the forward diffusion process. Following latest advances~\cite{dhariwal2021diffBeatGANs}, diffusion models achieve state-of-the-art performance, outperforming other classes of generative models, such as Generative adversarial networks (GANs), VQ-VAE~\cite{razavi2019VQVAE2}, and Autoregressive models~\cite{child2019sparseTransformer} on various metrics in image fidelity and diversity~\cite{nichol2021improvedDdpm, dhariwal2021diffBeatGANs}. Some of the key factors behind their success are the innovation on the architecture of the diffusion models~\cite{ho2020denoisingdiffusion, dhariwal2021diffBeatGANs}, simplified formulation for the training objective~\cite{ho2020denoisingdiffusion}, and use of cascaded diffusion processes~\cite{nichol2021improvedDdpm, dhariwal2021diffBeatGANs, ho2021cascadedDiffusion}.

Sampling from diffusion models is quite slow since it requires an iterative denoising operation. Reducing this overhead by developing fast sampling techniques is a topic of tremendous research interest~\cite{song2020ddim, jolicoeur2021gottaGoFast, kong2021fastSampleDDPM, watson2021LearnEfficientSampleDDPM}. Orthogonal to this direction, our interest is in sampling data from low-density neighborhoods. We further show that our sampling approach can be easily integrated with fast sampling techniques.

To measure neighborhood density around a sample, we use the Gaussian model of training data in the embedding space of a pre-trained classifier. Modeling images in embedding space is a common approach, particularly due to their alignment with human perception~\cite{zhang2018Lpips}, in numerous vision applications, such as outlier detection~\cite{sehwag2020ssd} and instance selection~\cite{devries2020instanceSelection}.

Across generative models, given a distribution learned by the model, there have been previous attempts in sampling from a targeted data distribution. Discriminator rejection sampling (DRS) and its successors \cite{azadi2018DRSGan, ding2020subsampleGANImfinetune} consider rejection sampling using the discriminator in a generative adversarial network (GAN). Similarly, Razavi~\etal~\cite{razavi2019VQVAE2} exploits a pre-trained classifier to reject samples that are classified with low confidence. Most often the goal is to filter out low fidelity samples, thus improving the quality of synthetic data. In contrast, our goal is to generate high fidelity samples from low-density regions of the data manifold. These samples are rarely generated by the model under uniform sampling, thus sampling them using a naive classifier-based rejection sampling approach leads to high-cost overheads. We instead opt to modify the generative process of diffusion models to guide it towards low-density neighborhoods of the data manifold.

The most closely related work to ours is from Li~\etal\cite{li2020ClassEmbedSmoothGAN}, which smoothes class embeddings of a BigGAN model to generate diverse images. In contrast, we focus on diffusion-based generative models. We also demonstrate the limitation of their approach with diffusion models in Appendix~\ref{app: SmoothEmbed}.







==> Diverse sampling from generative models [CVPR 22]/sections/methods.tex <==
In this section, we first provide an overview of the sampling process in diffusion-based generative models. Next, we describe our modification in the sampling process for low-density sampling. 

\subsection{Overview of diffusion models}
% \noindent \textit{Notation.}
% $p(.)$ to denote a probability distributions 
% \dummytext{5}
\vikash{First define the task of learning model distribution from the data distribution.}
Denoising diffusion probabilistic models (DDPM)~\cite{ho2020denoisingdiffusion} model the data distribution by learning the reverse process (generative process) for a forward diffusion process. The forward process is often a Markov chain with Gaussian transitions,~\ie, $q(\rvx_t|\rvx_{t-1}) := \gN(\rvx_t; \sqrt{1-\beta_t}\rvx_{t-1}, \beta_t\mathbf{I})$. Given a large number of timesteps ($T$), this diffusion process sufficiently destroys the information in input samples ($\rvx_0$) such that $p(\rvx_T) := \gN(\rvx_t; \mathbf{0}, \rmI)$.

Reverse or generative process is also assumed to be a Markov process with Gaussian transitions that learns the inverse mapping,~\ie, $p(\rvx_{t-1} | \rvx_t)$, at each time step. This process is usually modeled with a deep neural network, parameterized by $\theta$, that learns the Gaussian transition such that $p_\theta(\rvx_{t-1} | \rvx_t) := \gN(\rvx_{t-1}; \bm{\mu}_\theta(\rvx_t, t), \mathbf{\Sigma}_\theta(\rvx_t, t))$. \vikash{Bold mu in equations.} 
\begin{align}\label{eq: base_nll}
    p_\theta(\rvx_0) = p(\rvx_T) \prod_{t=1}^{T} p_\theta (\rvx_{t-1}|\rvx_t)
\end{align}
The model is trained by maximizing the variational lower bounds on the negative log likelihood over the training data.

In order to sample synthetic data from diffusion models, we first sample a latent vector $\rvx_T \sim \gN(\mathbf{0}, \mathbf{I})$ and iteratively denoise it using the following procedure in reverse process.
\vspace{-15pt}
\begin{align}
    \rvx_{t-1} = \bm{\mu}_{\theta}(\rvx_t, t) + \mathbf{\Sigma}_{\theta}^{1/2}(\rvx_t, t)\rvz,~~~~\rvz \sim \gN(\mathbf{0}, \mathbf{I})
\end{align}

We refer to this approach as \textit{baseline} sampling process.

\subsection{Generating synthetic images from low-density regions on the data manifold}
In this section, we present our approach to generating samples from low-density regions of data manifold using diffusion-based models.

\subsubsection{Identifying low-density regions on data manifold}
Given a data distribution $q(\rvx)$, low-density regions or neighborhoods are part of the data manifold that have significantly lower sample density than the others. To develop techniques to sample from these regions, the first step is to characterize them.

\textit{Limitation of likelihood estimates from the diffusion model.} A natural choice to characterize manifold density is to use the likelihood estimate from the diffusion model itself (Equation~\ref{eq: base_nll}). After all, we expect the likelihood of getting a sample from high-density regions being higher than the low-density regions. However, due to its intractability for diffusion-based models, the likelihood estimates from the model are only an approximation of exact likelihood~\cite{sohl2015NonEqDDPM,ho2020denoisingdiffusion}. We find that these likelihood estimates are not a reliable predictor of manifold density as they fail to align with multiple commonly used metrics or with human judgment (Appendix~\ref{app: diffLikelihood}).
This trend aligns with a similar limitation of likelihood estimates in autoregressive models~\cite{nalisnick2018GenDontKnow}. 

We shift our focus to discriminative models since they are well-known to learn meaningful embeddings that align with human perception for images~\cite{zhang2018Lpips}. We measure the manifold density by estimating the likelihood of data in the embedding space. Let $(g \circ f)(.)$ be a discriminative model, where $f$ extracts embeddings for the input image and $g$ is the head classifier, most often a linear model. We model embeddings of each class using a Gaussian model and estimate the log-likelihood of a given image ($\rvx_i$) with class label $\rvy_i$ from this model. We refer to the negative log-likelihood as \textit{Hardness score ($H$)}. 
% to break equation and use /left-\right. Using breakeqn package
% \begin{dmath}
%     H(\rvx, y) = \frac{1}{2} \left[\left(f(\rvx) - \mu_y\right)^T\Sigma_y^{-1} \left(f(\rvx) - \mu_y\right) \\ + \ln\left(\text{det}(\Sigma_y)\right) + k\, \ln (2\pi) \right]
% \end{dmath}
\vspace{-5pt}
\begin{align}
    \begin{split}
        H(\rvx, y) = \frac{1}{2} \Bigl[\bigl(f(\rvx) &- \mu_y\bigr)^T\Sigma_y^{-1} \bigl(f(\rvx) - \mu_y\bigr) \\ &+ \ln\bigl(\det(\Sigma_y)\bigr) + k\, \ln (2\pi) \Bigr]
    \end{split}
\end{align}

$\mu_y$ and $\Sigma_y$ refer to sample mean and sample covariance for embeddings of class $y$ and $k$ is the dimension of embedding space. We provide further analysis in Appendix~\ref{app: hardnessJustify} to justify that the decrease in manifold density leads to an increase in hardness score.

To sample from low-density regions, our approach is to guide the diffusion model to generate samples with high hardness scores,~\ie, equivalent to achieving low likelihood in the correct class. We maximize the following contrastive guiding loss for this task.
\vspace{-5pt}
\begin{equation}
    L_{g_1} (\rvx_i, y_i)  = \textnormal{log}\left[\frac{exp(H(\rvx_i, y_i)/\tau)}{\sum_{j=1}^{C}exp(H(\rvx_j, j)/\tau)}\right]
\end{equation}
where $\tau$ is the temperature and $C$ is the total number of classes. \vikash{Fix the notation issues in this section.}

This formalization of guiding loss function is fairly similar to cross-entropy loss on output softmax probabilities,~\ie, $(g \circ f)(.)$. Thus we also consider an equivalent loss function where instead of hardness score, we minimize the output softmax probability in the correct class.
% Instead of embedding space, we can also use optimize output softmax probabilities from the model. In particular, the negative softmax probability will be equivalent to the hardness score in the aforementioned loss function. 

\smallskip
\noindent\textbf{Incorporating guiding loss in sampling process.} The next step is to guide the sampling process to low-density regions by minimizing the log-likelihood of generated samples at each time step. We modify the sampling process as follows.
\vspace{-5pt}
\begin{align}\label{eq: sample_alpha}
\begin{split}
    \rvx_{t-1} = \bm{\mu}_{\theta}(\rvx_t, t) &+\, \mathbf{\Sigma}_{\theta}^{1/2}(\rvx_t, t)\, \rvz\\
    &+ \alpha\, \mathbf{\Sigma}_{\theta}(\rvx_t, t)\, \mathbf{\nabla}^*L_{g_1}(\rvx_{t}, y)
\end{split}
\end{align}
where $\rvz \sim \gN(\mathbf{0}, \mathbf{I})$, $\nabla^*$ refers to normalized gradients, and $\alpha$ is a scaling hyperparameter. We normalize gradients to disentangle the choice of scaling hyperparameter, $\alpha$, from the diffusion process time steps, $t$ (Appendix~\ref{app: normalGrad}). This formulation of sampling process is similar to Dhariwal~\etal~\cite{dhariwal2021diffBeatGANs}, with the modification that our loss function is designed to guide towards low-density regions and that we use normalized gradients. 

\subsubsection{Maintaining fidelity when minimizing likelihood}
We find that the sampling process in Equation~\ref{eq: sample_alpha} is highly successful at smaller values of $\alpha$. However, with higher values of $\alpha$, the guidance term dominates the Gaussian transition term from the diffusion model and steers the sampling process off data-manifold, thus generating very low fidelity images (as illustrated in Figure~\ref{fig: overview_steer}). Its effect is exacerbated by model distribution often not being a good approximation of data distribution in low-density regions, in particular, due to the reason that a very limited number of training samples are available from low-density regions.
\vspace{-10pt}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.9\linewidth]{images/overview.jpeg}
    \caption{An illustration demonstrating that small $\alpha$ values successfully guide the sampling process to low-density regions (lighter colors) on the data manifold. However, at large values of $\alpha$, using additional guidance (by using a non-zero $\beta$) from the binary discriminator (Eq.~\ref{eq: final_sampling}) helps in staying close to data manifold. We provide a demonstration of it in figure~\ref{fig: a_b_grid}.}
    \vspace{-10pt}
    \label{fig: overview_steer}
\end{figure}

We include another term in the sampling process to compel it to stay close to the data manifold. In particular, we train a binary discriminator, with hardness score $H'$, that distinguishes between synthetic and real samples. While sampling, we enforce synthetic images to stay close to the real data manifold by maximizing the following loss value. 
% \vspace{-5pt}
\begin{equation}
    \vspace{-5pt}
    L_{g_2} (\rvx_i)  = -\textnormal{log}\left[\frac{exp(H'(\rvx_i, 1)/\tau)}{\sum_{j=0}^{1}exp(H'(\rvx_j, j)/\tau)}\right]
\end{equation}
Here class zero and one represents synthetic and real images, respectively. In low-density regions, where model distribution is likely a poor approximation of real data distribution, this objective forces the diffusion model to generate samples that are closest to the real data manifold. Our final sampling process is following.
% If synthetic and real data is indistinguishable, adding this discriminator will have no effect. However, in low-density regions, where model distribution is likely distinguishable from real data distribution, this discriminator forces the model to generate samples that are closest to real data manifold. We modify the sampling process as follows.
% As shown in Figure~\ref{fig: overview_steer}, higher values of $\alpha$ steer the sampling process off data-manifold, thus generating very low fidelity images.
\vspace{-5pt}
\begin{align} \label{eq: final_sampling}
\vspace{-5pt}
\begin{split}
    \rvx_{t-1} = \bm{\mu}_{\theta}(\rvx_t, t) &+ \mathbf{\Sigma}_{\theta}^{1/2}(\rvx_t, t)\,\rvz\\
    &+ \alpha\, \mathbf{\Sigma}_{\theta}(\rvx_t, t)\, \mathbf{\nabla}^* L_{g_1}(\rvx_{t}, y)\\
    &+ \beta\, \mathbf{\Sigma}_{\theta}(\rvx_t, t)\, \mathbf{\nabla}^* L_{g_2}(\rvx_{t})
\end{split}
\end{align}

\vikash{Highlight that we refer to both loss terms as guidance loss function.}

where $\rvz \sim \gN(\mathbf{0}, \mathbf{I})$, $\nabla^*$ refers to normalized gradients, and $\alpha, \beta$ are scaling hyperparameters. To further demonstrate the combined effect of $\alpha$ and $\beta$, we provide synthetic images with a grid search over both hyperparameters in Figure~\ref{fig: a_b_grid}. We also detail our final approach in Algorithm~\ref{alg: final}.

\SetKwComment{Comment}{/* }{ */}
\begin{algorithm}
% \vspace{-10pt}
\caption{Sampling from low-density
regions.}\label{alg: final}
$\mathbf{Input:}~\textnormal{Class label}~(y), \alpha, \beta$\\
$\mathbf{Function:}~Normalize~(\rvu): \textnormal{return} ~\rvu/\norm{\rvu}$ \\
$\rvx_T \sim \gN(\mathbf{0}, \mathbf{I})$\\
\For{$i\gets T$ \KwTo \textnormal{1}}{
    \eIf{$t >$ \textnormal{1}}{
        $\rvz \sim \gN(\mathbf{0}, \mathbf{I})$, $\rvs \gets \mathbf{I}$
        
      }{
        $\rvz \gets \mathbf{0}$, $\rvs \gets \mathbf{0}$
      }
    $\rvu_1 = \alpha\, \mathbf{\Sigma}_{\theta}(\rvx_t, t)\, Normalize\left(\mathbf{\nabla} L_{g_1}\left(\rvx_{t}, y\right)\right)$\\
    $\rvu_2 = \beta\, \mathbf{\Sigma}_{\theta}(\rvx_t, t)\, Normalize\left(\mathbf{\nabla} L_{g_2}\left(\rvx_{t}\right)\right)$\\
    $\rvx_{t-1} = \bm{\mu}_{\theta}(\rvx_t, t) + \mathbf{\Sigma}_{\theta}^{1/2}(\rvx_t, t)\, \rvz  + \rvs (\rvu_1 + \rvu_2)$
}
\Return $\rvx_0$
\end{algorithm}










==> Diverse sampling from generative models [CVPR 22]/sections/rel_work.tex <==
We discuss papers from each related domains to ours. Since we already devote a significant space to background of diffusion models in methods, its not wise to put related work at the start. Otherwise it will be already 3-4 pages before the reader arrives at our core contributions. Anyway we aren't advancing our previous work, since this work is pretty tangential to most previous paper in generative modelling. 

\noindent \textbf{Diffusion based generative models.} This includes details on diffusion models. Few lines of how they are better than other generative models. \dummytext{4}

\noindent \textbf{Sampling techniques from generative models.} 
Discuss top-k sampling in VAE papers, Bean search and nucleus sampling in language models (GPT papers).
\dummytext{6}

\noindent \textbf{Synthetic-to-real domain transfer.} \dummytext{5}

\noindent \textbf{Robustness to domain-shifts.} \dummytext{6}

\noindent \textbf{Miscellaneous.} \dummytext{2}


\section{Further discussion}
\begin{itemize}
    \item There have been previous work on GANs on diverse sampling. Since all of us just uses a fixed generative model but modifies the procedure, it matter how good is generative model. As we show, ddpm models are better than gans, thus making our work of prime importance. But lets also make sure that it doesn't look like that we are doing an incremental work (since ddpm model has very novel challenge than gans). Lets discuss this previous work early on (like whats hiding in our networks paper).
    \item When comparing timing cost, also compare with cost when using fast sampling criterion. But argue that our techniques can be used with fast samplers too. 
    \item Lets focus on insights, even before jumping to applications. What hidden in the generative model?  If the data manifold modelled well for all classes.  I mean can it generate hard images well for all classes? If not then why not?
    \item Fig. 1 is main pitch. Put biggan, ddpm, and ours images. GANs can't do much due to poor coverage. DDPM model is much better (as we will also show) and we improve its ability a lot. 
    \item How about we also incorporate these images in our framework on proxy distributions. The might further boost the performance of adversarial training. 
    \item We might also need to retrain the diffusion models for some ablation studies, i.e., why did the diffusion network modelled low-density manifold so well? Will even limited number of samples from these regions make it worse?
    \item In memorization, do a very water tight analysis. Calculate pairwise distance (with 1M synthetic and 1M real images) and flag images that are super close to each other. 
    \item Are these examples adversarial? No, as slight variation in objective leads to perceptible changes, not adversarial ones.. Even if there are some, we choose to use a different network in our analysis (resnet50) than one used in optimization.
    \item How about we use a toy experiment like using mixture-of-Gaussian to explain our idea a bit more intuitively (something like \url{https://openreview.net/pdf?id=lsQCDXjOl3k}).
    \item Compare with VQGAN too when arguing about use of diffusion based models. BigGAN comparison just seems to naive and will invite further criticism.
    \item Before applications, add another section on analyzing low-density samples. We analyze 1) if the network is simply memorizing them 2) the intriguing transformation network exploit to generate them 3) Some likelihood to verify that they are low-density (don't use classifier to do it)
    \item Arange related work in 1) Selective sampling (Discriminator Rejection Sampling, VAE and many others for high fidelity, LOGAN and other for high diversity). 2) Benefit of synthetic data (in benign and adversarial training). Ideally humans are best for rejecting/accpeting samples (as argued in future work of discriminator rejection sampling paper).
    \item Why don't we also use a discriminator (like discriminator rejection sampling) to make sure that we stay close to the real data distribution. Say random sampling lead to true distribution but higher $\alpha$ led to much different distribution. We might have moved too far from real-data distribution then. We need to ensure that it doesn't happen. This could serve as an visualization of our approach. 
    \item Use concrete terms like top-k sampling, nucleus sampling and provide comparison with them.
    \item We also uncovered that some classes for the dataset have much less coverage of the distribution that others, since the fidelity of images quickly degraded.
    \item Compare with other related papers that are under submission at ICLR. 
    \item Its not hard instances that we are after. True our framework can generate both easy and hard instances. Hard instances is also a vague term. What we specifically are optimizing for is to generate rate to occur samples from training data. Even more samples that are absent from training data, but somehow the generate model construct them out of nowhere. 
    \item To motivate the problem, we can first show both high and low-likelihood images in training set. GAN are known to not model low-likelihood. Diffusion model seems to do it but random sampling doesn't suffice. We develop techniques to sample low-likelihood images from diffusion based models. So spli figure 1, real images into two. Keep some space between Real and others.
    \item Generate some 512x512 images for visualization.
    \item Again Hardness is very subjective metric. Lets tick to using likelihood as a measure of whether the sample belong to low-density region of the distribution.
    \item Goal to meet: You must make your paper easy to read. You've got to make it easy for anyone to tell what your paper is about, what problem it solves, why the problem is interesting, what is really new in your paper (and what isn't), why it's so neat.
    \item How training on low density data helps. How about we train on synthetic (random vs ours) and test on real (training set since test set doesn't have enough images). There can our approach slow down the rate at which accuracy degrades (even if it start at a smaller accuracy for easier images). 
    \item To constructively demonstrate the impact of both loss terms, lets display a grid. Starting from one image, change one coefficient on one axis and another coefficient. Do it for 3-5 images, keep one in the main paper and rest in the appendix.
    \item Lets try to follow a similar presentation style as original StyleGAN paper: https://arxiv.org/pdf/1812.04948.pdf
    \item To compare with random sampling (in training aspect), we can use a use a dataset which is unformly distributed, unlike a long-tail distribution like real data or random sampling. 
    \item Motivation in methods section. Mention that in low-density regions, not much samples are available, thus the generative distribution may lie far away from real data distribution. Its most critical that we use a guidance term there. It will become evident from our plot that this additional loss term has most impact when the distance from the centroid of the manifold is highest.
    \item Lets stick to only a few things in the analysis: Memorization and class-wise discrepancy and that's all. Too much content leads to much high exposure.
    \item A baseline for us could be the Nyguen paper on BigGAN diverse sampling or LoGAN. Both are both GANs, which are totally different from Diffusion models. Nevertheless, we try the class-condition smoothing idea but find that diffusion model doesn't respond very well and quickly generates poor quality images. In contrast our approach work very well. 
    \item Put the results on OOD robustness in the appendix of the paper (since we don't have a conclusive trend there). 
    \item We argue that for low-density sample the model quickly generated bad samples. What would be analogy in terms of scores. Are score in low-density region not define well (due to lack of data) and thus not learned well.
    \item By default the model is trained to maximize the likelihood (or lower bound) at each transition. Our approach allows us to guide model toward low-likelihood, but still on-manifold regions. \item Though we are first to try this idea on ddpm, lets compare with a few baselines on ddpm itself: 1) with class smoothing 2) optimizing on x-start instead of x-t in the diffusion process. 
    \item Note that our samples are continuous in the diffusion process, so we can't talk about their point probabilities (only true for x-start which is discrete). Also likelihood core definition that it is regarded as the likelihood of a set of parameters give outcomes. So its more natural to talk about likelihood when optimizing parameters (since its parameters likelihood that we are optimizing, give observed values). But it doesn't make sense to talk about instance likelihood. 
    \item How do we argue that the model is biased to sample from high-density region, as more data is centered there. 
    \item Contrast out approach with interpolation in low-density space, i.e., from where no novel images are seen at training time, such as work on Dall-E.
    \item Lets also add a section where we compare the density of generated samples using other distance metrics, such as k-nn, likelihood, changing representation spaces etc.  
    \item Discuss Vitaly Feldman's paper on long tale, which argues the its necessary to memorize low-density data otherwise the network may not generalize there. 
    \item Make sure to include coverage of distribution from multiple other metrics, such as recall, k-nn neighbors etc. 
    \item To address limitation of our method to supervised setting, also add another section of using contrastive learning based loss for unsupervised setting (assuming a supervised classifier is available). 
    \item Contrast to ML paper, follow style of a common CVPR paper: \url{http://selfcondgan.csail.mit.edu/preprint.pdf}. Similar to their fig. 4, add visual examples comparing our approach with uniform sampling and real images. 
    \item In appendix add a comparison section of different likelihood esitmation metric. Take 20 images from an easy class from ImageNet and sort them based on each of the metric. See which metric do well and which don't. May be add some basic negative too (like white noise, all-black pixel images etc to test the robustness). We can refer to this plot to justify why we didn't optimize the model likelihood and why we choose the embedding space to optimize.
    \item To justify why higher alpha makes things worse since model distribution is not accurate, plot the results with minimizing negative log-likelihood and show that there the model can sustain much higher values of alpha but not in the other direction.
    \item Address the selective vs random picking of visual examples. 
    \item Use visualization with the images generated from the embedding loss, instead of soft-max loss (even though they are mostly equivalent). 
    \item One might ask, how high is the fidelity of our generated samples? Well that's hard to answer, since existing generative models have trouble generalizing to them.
    \item Can we also show that our work can be further integrated with ddim and other fast sampling approaches?
    \item Make sure to include demo images from CIFAR-10 dataset too, otherwise we will be shot-down for just using one dataset.
    \item Discuss the instability in the inverse of covariance matrix at higher time stamps. We need to talk about it in the experimental setup section or the methods itself. Note that this is only the case for optimization. As inference, when t=0, we do consider sigma without any approximation. 
    \item We also need to discuss the selection procedure for alpha and beta, in particular when selecting images for some applications.
    \item 
\end{itemize}
% Why we don't end up generating adversarial examples.


==> Diverse sampling from generative models [CVPR 22]/sections/results.tex <==
\begin{figure}[!b]
    \centering
    \includegraphics[width=\linewidth]{images/alpha_beta_grid_1_256.pdf}
    \caption{\textbf{Controlling hardness and fidelity.} Effect of increasing $\alpha$ (y-axis) and $\beta$ (x-axis) on synthetic images. Increasing $\alpha$ forces the model to sample from low-density regions while $\beta$ forces the sampling process to stay close to real data manifold. Salient impact of $\beta$ includes improving foreground semantics to correctly represent the class and preserving background information.}
    \label{fig: a_b_grid}
\end{figure}

% \begin{figure*}[!btp]
%      \centering
%      \begin{subfigure}[t]{0.49\textwidth}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/baseline_class_0.png}}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/ours_class_0.png}}%
%         \vspace{7pt}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/baseline_class_7.png}}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/ours_class_7.png}}
%         \caption{ImageNet (class 0 and 7)}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\textwidth}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/baseline_class_82.png}}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/ours_class_82.png}}%
%         \vspace{.6ex}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/cifar10_baseline_samples.png}}
%         \raisebox{-\height}{\includegraphics[width=0.49\textwidth]{images/cifar10_ours_samples.png}}
%         \caption{ImageNet (class 73) and CIFAR-10}
%     \end{subfigure}
%     \caption{Comparing synthetic images from the baseline sampling process (left) and our approach (right). We use the identical randomness seed for both approaches. Therefore, each pair of images among two approaches start from the identical latent vector and the only difference is being the additional guidance term in our approach. [Plot cifar images separately., plot 3x3 image grid for more clarity. It cluttered right now. May be show only two classes for cifar-10, but 6x6 grid for each. Put a 4x4 grid in appendix., Refer to progressive plots in Discussion.]}
%     \label{fig: add_demo_images}
% \end{figure*}


\noindent\textbf{Experimental setup.}
We use a U-Net-based architecture with adaptive group normalization for the diffusion model~\cite{dhariwal2021diffBeatGANs}. We consider the encoder from U-Net for the classifier architecture. Both classifier and diffusion model are conditioned on the diffusion process timestep. We consider $T=1000$ for the diffusion process. When sampling, we use $250$ timesteps, as it speeds up the sampling process while incurring negligible cost in the image quality.


\begin{figure}[!b]
    \vspace{-10pt}
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=\linewidth]{images/hardness_vs_alpha.pdf}
        \caption{$\alpha$ increases the hardness score.}
        \label{fig: ablate_alpha}
    \end{subfigure}
    \hspace{10pt}
    \begin{subfigure}[b]{0.45\linewidth}
        \includegraphics[width=0.9\linewidth]{images/prec_vs_beta.pdf}
        \caption{$\beta$ improves the fidelity}
        \label{fig: ablate_beta}
    \end{subfigure}
    \vspace{-5pt}
    \caption{\textbf{Validating effect of hyperparameters.} Quantitative results validating the desired effect of hyperparameters $\alpha$ and $\beta$. }
    \vspace{-15pt}
\end{figure}


\begin{figure*}[!btp]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
        \raisebox{-\height}{\includegraphics[width=\linewidth]{images/samples_ours_class_900.jpeg}}%
        \vspace{10pt}
        \raisebox{-\height}{\includegraphics[width=\linewidth]{images/samples_baseline_class_900.jpeg}}
        \caption{Water tower}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \raisebox{-\height}{\includegraphics[width=\linewidth]{images/samples_ours_class_400.jpeg}}%
        \vspace{10pt}
        \raisebox{-\height}{\includegraphics[width=\linewidth]{images/samples_baseline_class_400.jpeg}}
        \caption{Academic robe}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \raisebox{-\height}{\includegraphics[width=\linewidth]{images/samples_ours_class_300.jpeg}}%
        \vspace{10pt}
        \raisebox{-\height}{\includegraphics[width=\linewidth]{images/samples_baseline_class_300.jpeg}}
        \caption{Tiger beetle}
    \end{subfigure}
    \vspace{-5pt}
    \caption{\textbf{Comparing samples from proposed and baseline sampling process.} We compare synthetic images from our proposed sampling approach (top) with the baseline sampling process (bottom) on the ImageNet dataset. We use identical random seed for both stochastic sampling processes. Therefore, generation of each pair of images among the two approaches starts from the identical latent vectors and the only difference is the additional guidance terms in our approach.}
    \label{fig: add_demo_images_imagenet}
\end{figure*}


\begin{figure*}[!btp]
     \centering
    \begin{subfigure}[t]{0.48\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.48\linewidth]{images/samples_cifar10_baseline_class_1.jpeg}}%
        \hspace{5pt}
        \raisebox{-\height}{\includegraphics[width=0.48\linewidth]{images/samples_cifar10_ours_class_1.jpeg}}
        \caption{Automobile}
    \end{subfigure}
    \hspace{10pt}
    \begin{subfigure}[t]{0.48\textwidth}
        \raisebox{-\height}{\includegraphics[width=0.48\linewidth]{images/samples_cifar10_baseline_class_9.jpeg}}%
        \hspace{5pt}
        \raisebox{-\height}{\includegraphics[width=0.48\linewidth]{images/samples_cifar10_ours_class_9.jpeg}}
        \caption{Truck}
    \end{subfigure}
    \vspace{-5pt}
    \caption{\textbf{Comparison on CIFAR-10 dataset.} We compare synthetic images from the baseline sampling process (left) with our proposed sampling approach (right) on the CIFAR-10 dataset. We use the identical seed for random number generators for both processes.}
    \vspace{-10pt}
    \label{fig: add_demo_images_cifar10}
\end{figure*}

We consider two commonly used image datasets: CIFAR-10~\cite{krizhevsky2009learning} and ImageNet~\cite{deng2009imagenet}. When training the binary discriminator, $H'$, we first uniformly sample synthetic images equal to the size of the training dataset,~\ie, $50$K images for the CIFAR-10 dataset and $1.2$M images for the ImageNet dataset. We conduct a hyperparameter search for $\alpha$ and $\beta$ between $0.01$ and $1.0$. In most analyses, we sample $50$K synthetic images for ImageNet and $10$K synthetic images for the CIFAR-10 dataset, i.e., equal to the size of validation set for each dataset. We provide additional experimental details in Appendix~\ref{app: setup}. 

When sampling we optimize the likelihood estimate,~\ie, hardness score, calculated in the embedding space of the U-Net encoder model. To measure generalization to other representation spaces, we consider multiple other models to calculate hardness scores post sample generation. We present results with the ResNet-50 model in the main paper and the rest in the Appendix~\ref{app: kNNClassifier}.
\vikash{Add details on the cascading model and that we only for the smallest resolution.}

\vikash{Add the controlled experiment to demonstrate the success of our approach.}
% Once complete, this section will include a small-scale experiment where we have a control on low-density regions of the distribution. In this setup, we show that our approach finds these low-density regions, something uniform sampling rarely picks.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.3\linewidth}
         \includegraphics[width=\linewidth]{images/hardness_score_model_comparison.pdf}
          \caption{Hardness score}
    \end{subfigure}
    \hspace{10pt}
    \begin{subfigure}[b]{0.3\linewidth}
         \includegraphics[width=0.92\linewidth]{images/5NN_distance_model_comparison.pdf}
         \caption{AvgkNN distance}
    \end{subfigure}
    \begin{subfigure}[b]{0.3\linewidth}
         \includegraphics[width=0.97\linewidth]{images/local_outlier_factor_k_20_model_comparison.pdf}
         \caption{Local outlier factor}
    \end{subfigure}
    \vspace{-5pt}
    \caption{\textbf{Comparing neighborhood density.} We measure the density in the neighborhood of a given set of instances using three different metrics. All three metrics share a common trend: while baseline sampling generates synthetic samples that have similar density distribution as real data, our sampling process generates samples from low density neighborhoods with higher probability.}
    \label{fig: density_comp}
    \vspace{-10pt}
\end{figure*}

\subsection{Generating synthetic data using proposed $\alpha \text{-} \beta$ guided sampling process} \label{sec: alpha_beta_results}
\noindent \textbf{Validating the effect of hyperparameter $\alpha$ and $\beta$.} 
Our sampling process is designed such that we can sample images from the low-density regions by increasing $\alpha$ and improving the fidelity of these images using $\beta$. Our first goal is to validate the desired effect of both hyperparameters.

While using $\beta=0$, we first increase $\alpha$ value from $0$ to $1.0$ and measure the hardness score of sampled images at each value (Figure~\ref{fig: ablate_alpha}). Our results demonstrate that increasing $\alpha$ shifts the hardness score distribution to the right, i.e., higher probability of sampling images that have lower estimated likelihood.
% getting a sample images with lower likelihood. 

Next we fix $\alpha=0.5$ and increase $\beta$ from zero to two. We use precision~\cite{sajjadi2018PrecisionRecall} to measure the fidelity of synthetic images. It broadly measures the fraction of images that are realistic or equivalently, the coverage of synthetic data by the support of training data distribution. Our results show that increasing $\beta$ does improve the realism of generated synthetic images (Figure~~\ref{fig: ablate_beta}).

Finally, we analyze the joint effect of parameters $\alpha$ and $\beta$. We perform a grid search over both $\alpha$ and $\beta$ and generate images for each pair of values. To avoid the impact of stochasticity, we use the same seed for all runs of the sampling process. We present the sampled images in Figure~\ref{fig: a_b_grid}. 

These visualizations validate our argument that solely increasing $\alpha$ to very high values degrades image fidelity. This is because a higher value of $\alpha$ encourages sampling of low-likelihood images. However, the model can satisfy this constraint by simply generating a poor-quality image. Increasing $\beta$ addresses this issue, in particular on high values of $\alpha$,  where it restores the key attributes of the image thus effectively moving it closer to the data manifold. We find that a $1:1$ ratio between $\alpha$ and $\beta$ strikes a modest trade-off between sample hardness and fidelity and use $\alpha=\beta=0.5$ for further experiments.

% \textbf{Guiding principles for choice of $\alpha$ and $\beta$.} Provide some recommendation on how to choose these two values.  



% \noindent\textbf{Additional visualization comparison of our samples with baselines.} 
% Following our earlier grid search, we set $\alpha$ and $\beta$ to $0.05$ and $0.1$, respectively, for the ImageNet dataset. We find that similar values of hyperparameter are also effective for the CIFAR-10 dataset.

\noindent \textbf{Comparing our sampling process with the baseline sampling process.}
 We compare the synthetic images generated from the baseline and our sampling approach in Figure~\ref{fig: add_demo_images_imagenet},~\ref{fig: add_demo_images_cifar10}. We use identical experimental setup, including seeds for random number generators, for both sampling processes thus leaving guidance terms to be the only factor impacting final images. Images from our approach are visually distinguishable from the baseline approach since the diffusion model introduces significant changes in the foreground object semantics and background to satisfy the constraints on hardness and fidelity. We provide additional visualizations in Appendix~\ref{app: sampleComp}. 

\subsection{Quantitative comparison of neighborhood density}
To validate that our sampling process does generate data from low-density regions, we quantitatively compare the manifold density in the neighborhood of synthetic images with different baselines. 


\noindent \textbf{Metrics to measure neighborhood density.} We use hardness score as the first validation metric since we maximize it in the sampling process. However, our sampling process might maximize hardness score without actually moving the sampling process to low-density regions. Thus we consider two additional metrics, namely Average nearest neighbor (AvgkNN) and local outlier factor (LOF)~\cite{breunig2000lof} to further validate the success of our approach. AvgkNN measures density using proximity to nearest neighbors. We choose five nearest neighbors, which is a common choice~\cite{devries2020instanceSelection}. In contrast, the local outlier factor improves on the nearest-neighbor distance metric to compare density around a given sample to density around its neighbors. Higher values of the local outlier factor indicate the sample lies in a much lower density region than its neighbors. We calculate all distances in the feature space of a ResNet50 network which is pre-trained on the ImageNet dataset. We ablate on the choice of feature extractor in Appendix~\ref{app: kNNClassifier} and show that our conclusions don't change with this choice. For this analysis, we sample $50$K synthetic images using recommended values of $\alpha$ and $\beta$ from Section~\ref{sec: alpha_beta_results}. We compare our approach with three baselines 1) BigGAN-deep 2) Real images from the ImageNet validation set and 3) synthetic images generated using baseline sampling from the DDPM model. We present our results in Figure~\ref{fig: density_comp}. 

\noindent \textbf{All three metrics validate the success of our approach.} 
Under all three metrics, our sampling process has a higher probability of generating synthetic images from low-density neighborhoods. It also validates the claims that the sample density in real data itself follows a long-tail distribution and an unmodified sampling process, i.e., baseline sampling process, from diffusion models closely approximates this distribution. In comparison, BigGAN samples are predominantly from low-density regions. Among the three metrics, the difference between our approach and baseline is most significant in AvgkNN distance. When ablating on the choice of the guidance loss function, we find that under sufficient hyper-parameter ablation, one can obtain equivalent results when optimizing likelihood in embedding space or softmax probabilities after the logit layer (Appendix~\ref{app: tempEffect}).

\vikash{Add some details on the number of images used for each dataset. Do this for other sections too as such details are often missing.}

% All five metrics validate our claims that the proposed sampling process generates samples from low-density regions. It also validates the claims that the sample density in real data itself follows a long-tail distribution and an unmodified sampling process closely approximates this distribution. \\



% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.45\linewidth}
%          \includegraphics[width=\linewidth]{images/hardness_score_comparison_generative_model.pdf}
%           \caption{Hardness score}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.45\linewidth}
%          \includegraphics[width=\linewidth]{images/hardness_score_comparison_generative_model_ours.png}
%          \caption{Hardness score (ours) with different values of $\alpha$.}
%     \end{subfigure}
%     \caption{Comparing density of samples generated from our approach with density of uniformly sampled images. [We will soon add results with other metrics.]}
%     \label{fig: density_comp}
% \end{figure}

\begin{table}[!b]
    \centering
    \vspace{-20pt}
    \caption{\textbf{Reduction in sampling cost.} Comparing the sample generation time of our method with uniform sampling. Each entry represents the time taken (in days) to generate $5$K $256\times256$ resolution synthetic images from the corresponding hardness score range on a single A100 GPU.}
    \label{tab: cost_comp}
    \vspace{-5pt}
    \begin{tabular}{cccc}  \toprule
     Score-range & $200-240$ & $240-280$ & $280-320$ \\ \midrule
     Baseline & $1.99$ & $5.74$ & $16.79$ \\ 
     Ours & $1.88$ \scriptsize{($\times \textbf{1.1}$)}  & $2.03$ \scriptsize{($\times \textbf{2.8}$)} & $2.78$ \scriptsize{($\times \textbf{6.0}$)} \\ \bottomrule
     % [18.1 20.4 29.4] (scale=0.5), [17.2 28.  50.6] (scale=0.1), [16.9 23.6 37.3](scale=0.2), [18.  36.4 75.7](scale=0.05), [ 24.   67.7 187.2](scale=0.005)
    \end{tabular}
    % \vspace{-5pt}
\end{table}

\noindent \textbf{Equivalent reduction in computational cost.} Assume that we want to sample images from low-density neighborhoods,~\ie, the hardness score of each synthetic sample is greater than a threshold. A naive rejection sampling-based approach is to sample images uniformly at random and reject images that do not satisfy the criterion. However, due to the long-tail nature of sample density, the likelihood of a sample being from low-density regions is low, thus we would need to reject many samples to curate desired samples. Due to the iterative nature of the sampling process, generating synthetic data from diffusion models is computationally expensive, thus making rejection sampling a highly computationally costly approach (Table~\ref{tab: cost_comp}). Our approach does not depend on rejection sampling, thus it is up to $2-6\times$ faster than the former approach (Table~\ref{tab: cost_comp}). 
% \begin{figure*}[!htb]
%     \centering
%     \begin{subfigure}[b]{0.22\linewidth}
%          \includegraphics[width=\linewidth]{images/hardness_score_comparison_generative_model.pdf}
%           \caption{Hardness score}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\linewidth}
%          \includegraphics[width=\linewidth]{example-image-golden}
%          \caption{k-NN}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\linewidth}
%          \includegraphics[width=\linewidth]{example-image-golden}
%          \caption{Probablisitc-PCA}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\linewidth}
%          \includegraphics[width=\linewidth]{example-image-golden}
%          \caption{Recall}
%     \end{subfigure}
%     \caption{Comparing density of samples generated from our approach with density of uniformly sampled images. We use four different methods to measure neighbourhood density.}
%     \label{fig: density_comp}
% \end{figure*}



% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{images/progressive_hardness.png}
%     \caption{Progressive moving synthetic samples to low-density regions.}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_992.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_323.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_985.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_130.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_89.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_604.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_900.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_779.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \begin{subfigure}[b]{\textwidth}
%          \centering
%          \vspace{-10pt}
%          \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_0.jpeg}
%          \vspace{-10pt}
%     \end{subfigure}
%     \caption{Progressive hardening of samples. TODO: Also display hardness score below each image.}
% \end{figure*}

% \section{Further analyzing low-density synthetic samples}
\section{Is our sampling process generating memorized samples from training data?}
Since a limited number of samples are available from low-density regions in our long-tailed datasets, the generative model might memorize these samples and fails to generate novel samples from these regions. Therefore we conduct a rigorous analysis to identify whether our sampling process is exploiting any memorization that might be happening in diffusion models.
% \vikash{Again add our experimental details like how many images etc. }


% We argue that if training data is being memorized, synthetic images will be substantially similar to train data. For every synthetic image generated by our approach, we compute its nearest neighbor distance from real training images. We compare this distance with two baselines: 1) Nearest neighbor distance for real images in the validation set and 2) Nearest neighbor distance for synthetic images from baseline sampling. We measure the distance in the embedding space of a ResNet-50 network trained on ImageNet. We ablate this choice in Appendix xyz. 

\begin{figure}[!b]
    \centering
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{images/nearest_neighbor_pairs_ddpm_ours.png}
    \vspace{-10pt}
    \caption{\textbf{Is low-density synthetic data being memorized?} Pairs of synthetic and real images with smallest euclidean distance in the feature space. In each pair, left and right image correspond to synthetic and real image, respectively. Our search space for these examples includes all pairs of 50K synthetic images and 1.2M real images. While the synthetic images share multiple attributes with the nearest real image, they are not identical to the real images.}
    \label{fig: nn_pairs}
    \vspace{-20pt}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/nearest_neighbor_real_data.jpeg}
    \vspace{-10pt}
    \caption{\textbf{Is low-density synthetic data novel?} 
    For each synthetic image, we analyze the class label of five nearest neighbors from real data. While each synthetic image has high fidelity and correctly represents the class, it often lies closer to samples of other classes in feature space. Even when the class label is not different, the synthetic image differs significantly from closest real samples. \vikash{Ablate the choice of embedding network to avoid the critique that it's because of this network. Include bus in sky example.}\label{fig: nn_ours}}
    \vspace{-30pt}
\end{figure}

\noindent \textbf{Analyzing nearest-neighbor distance.} We argue that if training data is being memorized, synthetic images will be substantially similar to training data. We measure this similarity by euclidean distance in the embedding space of well trained image classifiers. Thus, if a synthetic image is simply memorized from training data, its nearest-neighbor distance from real data will be very small. 

We sample $50$K images using our sampling approach and measure their nearest neighbor distance from $1.2$M real images in the training set of the ImageNet dataset. We compare these values with the nearest neighbor distance for real data in the validation set. If our approach has memorized training samples, its nearest neighbor distance should be much smaller than real samples. However, the average distance for our samples is $0.42$, much higher than $0.29$ for real samples. It supports our hypothesis that our sampling process is not simply generating memorized training samples. 

\noindent \textbf{Analyzing synthetic-real data pairs for signs of memorization.} Moving beyond comparing distribution statistics, now we analyze individual samples for signs of memorization. In particular, our goal is to manually analyze synthetic images and their closest neighbors for signs of memorization. Even more, we want to analyze pairs that would have the highest likelihood of being memorized, i.e., synthetic samples which are closest to real data. Across all $60$B pairs ($50\text{K}\times1.2$M)  of synthetic and real images, we manually analyze the top-500 pairs with the smallest pairwise distance. 

We observe that while images in these pairs share multiple attributes, such as object shape, texture, and identity, they are not being memorized. Instead, they are some semantic variation of the real images, highlighting that the diffusion model learned the data manifold instead of memorizing these samples. We present the top twelve pairs in figure~\ref{fig: nn_pairs} and the rest of them in Appendix~\ref{app: kNNPairs}.  

\noindent \textbf{Novel samples from low-density regions.} To validate that our sampling process is indeed generating novel images from low-density regions, we also consider the class label of its nearest neighbors from real data. In multiple cases, we find that the nearest neighbors have different class label than the synthetic sample. We provide few such examples in Figure~\ref{fig: nn_ours}. This phenomenon likely arises due to poorly learned representation by the embedding extractor in low-density regions, primarily due to the scarcity of training samples in these regions.




% Quantitative experiment: Per sample wise distance. Manually analyze the pair of samples. Of course distance is measured from the training data. Our trend shouldn't be any different from real-real distance (otherwise memorization is happening). Do it for a couple of different networks to make sure that our conclusions are not biased. Do it for ImageNet and cifar-10.

% Real dataset itself is long-tailed, thus only have a limited number of low-density samples (refer to figure 1). Thus under limited samples, would these models be able to interpolate. Its is well established to generative models in language space ends up memorizing not so frequently occurring samples. 

% Despite having access to very small number of sample, we observe that the model successful interpolates in the low-density regions. We provide some evidence supporting this claim in Figure~\ref{fig: nn_ours}. We will further add more quantitative results. \dummytext{5}


% \subsection{It's not exploiting adversarial perturbations.}
% To sample hard instances we add gradients from a classifier to reduce the likelihood. It is well known that these gradients can also lead to generating adversarial examples (some reference on this happening in GANs). However, we find that the iterative nature of the sampling process diminishes the effect and overall the classifier gradients act as a semantic guide (more on it in the appendix). 

\section{Discussion}
We present an improved version of the sampling process in diffusion-based generative models that enables sampling from low-density neighborhoods of the data manifold. We achieve this by guiding the sampling process using two additional classifiers at each timestep. Our sampling process successfully generates novel samples from low-density regions. Our work also identifies another compelling advantage of diffusion models. Despite being trained on a small number of samples from low-density regions, diffusion models successfully interpolate in these regions, i.e., don't memorize the training data from these regions. 

We analyze the impact of our guiding loss by juxtaposing samples from baseline and our sampling process (Figure~\ref{fig: add_demo_images_imagenet},~\ref{fig: add_demo_images_cifar10}). These results demonstrate that the generative model exploits novel transformations in response to guiding loss objectives. We further analyze this effect, by progressively increasing $\alpha$ while keeping all other parameters fixed (Figure~\ref{fig: progress_sampling}). Higher values of $\alpha$ forces the model to generate low-likelihood samples. We find that the network sometimes exploits transformations such as photometric changes, zoom, viewpoint, and switching the background to reduce the likelihood of synthetic samples.

 % juxtapose sample from baselines sampling process and our modified version of it with guiding loss functions (Figure xyz). Using these results, we demonstrate that our sampling process guided baselines sampling process to low-density regions. 

% We conduct a controlled experiment where we progressively increase the $\alpha$ while keeping all other parameters fixed. At each value of $\alpha$ we generate a set of synthetic images and compare these semantic changes in these images. Higher values of $\alpha$ imply that the generated images will have lower likelihoods. We present our results in Figure~\ref{fig: progress_sampling}. We provide additional examples in Figure~\ref{} in Appendix xyz.

% \noindent\textbf{Which novel transformations does the model exploit?}
% Since the model is not memorizing training data in low-density regions, a natural question is to analyze the novel attributes present in these samples. We aim to analyze the novelty of these samples through the lens of image transformations, which the network might employ in addition to tweaking foreground object attributes. Our sampling process is unbounded,~\ie, the network is not constrained to minimize the log-likelihood of samples using a specific set of transformations. 

% We conduct a controlled experiment where we progressively increase the $\alpha$ while keeping all other parameters fixed. At each value of $\alpha$ we generate a set of synthetic images and compare these semantic changes in these images. Higher values of $\alpha$ imply that the generated images will have lower likelihoods. We present our results in Figure~\ref{fig: progress_sampling}. We provide additional examples in Figure~\ref{} in Appendix xyz.

% We find the network exploits transformations such as photometric changes (low lightning conditioning), zoom in or out of the image, and tweaking the background of the images. Since we use the embedding of a pre-trained classifier to measure likelihood, our sampling process might exploit the bias of this classifier. For example, it is well known that the \textit{tench fish class} images in ImageNet often include a human holding the fish. Supervised classifier picks up this bias and learns to correlate the output with the human in the background. We often observe that the generative model simply removes the human from the background, thus incurring a large effect on its embeddings due to the bias of the classifier. 

\begin{figure}[!tb]
    \centering
    \begin{subfigure}[b]{\linewidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_130.jpeg}
         \vspace{-10pt}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
         \centering
         \vspace{-10pt}
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_779.jpeg}
         \vspace{-10pt}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
         \centering
         \vspace{-10pt}
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_0.jpeg}
         \vspace{-5pt}
    \end{subfigure}
    \vspace{-30pt}
    \caption{\textbf{Progressive sampling.} We incrementally increase $\alpha$ across different runs of the sampling process. It highlights how the guiding loss progressively moves the synthetic images to low density regions.}
    \vspace{-20pt}
    \label{fig: progress_sampling}
\end{figure}
% Key things to highlights:
% 1. We aren't simply memorizing data. For harder images nearest samples are easier instances from data. Even if we don't plot it right now, at least save the hardness score of each of image in file name. 
% 2. 


The sampling process in diffusion models iterates for hundreds of steps to generate a single sample. This challenge is often solved using a fast sampling process, which trades off sample quality for speed~\cite{song2020ddim, jolicoeur2021gottaGoFast}. To demonstrate that our approach can also integrate with fast sampling techniques, we integrate our modified sampling process with the fast sampling approach from Song et al.~\cite{song2020ddim}. We find no strikingly different trade-off between fidelity and sampling steps for the baseline and our approach (Appendix~\ref{app: ddim}). At a very low number of sampling steps, such as ten, both approaches struggle to generate high-quality images. However, with increasing the number of timesteps, the fidelity of both baseline and our approach quickly improves.


% There is no strikingly different trade-off between fidelity and sampling steps for the baseline and our approach.
% One major limitation of diffusion based generative model is slow sampling speed, since the sampling process in diffusion iterates for hundreds of thousands of steps to generate a single sample. 

% \smallskip
% \noindent\textbf{Can we sample hard instances fast?}\\
% Sampling process in diffusion iterates for hundreds of thousands of steps to generate a single sample. To reduce this computational cost, recent works have introduced faster sampling techniques. We now test our modified sampling process with the fast sampling approach from DDIM~\cite{song2020ddim}. We integrate the guiding loss in the DDIM sampling process in a similar manner as Dhariwal~\etal~\cite{dhariwal2021diffBeatGANs}.

% Our goal is to analyze whether how the fidelity of low-density synthetic samples degrade with the reduction in the number of sampling steps and compare this with the baselines sampling process. We present this comparison in Figure~\ref{fig: ddim_comp}. We use identical initial latent vectors for both approaches. We also significantly reduce the value of hyperparameters $\alpha$ and $\beta$ to match the scale of residuals in each step of the DDIM sampling process. \vikash{how much?}

% There is no strikingly different trade-off between fidelity and sampling steps for the baseline and our approach. At a very low number of sampling steps, such as 10, both approaches struggle to generate a high-quality image. However, with increasing the number of time steps, the fidelity of both baseline and low-density synthetic samples quickly improves.

\section{Limitations and broader impact}
% Discuss that we navigate data manifold through a the feature space of image classifiers. While the feature distance correlate with human judgement, the classifier are known to have certain biases, such as texture, background. The sampling process might exploit these biases to satisfy our constraints in feature space. Class label is hard to control in this problem space.  Provide some failure cases in appendix. Future work is need to build more precise controls. 

% Unsupervised learning for future work. Note that we use the embedding of a pre-trained classifier to measure likelihood, thus our sampling process might exploit the bias of this classifier. We find 

We guide the sampling process by navigating the data manifold through the feature space of image classifiers. While proximity in feature space of deep neural networks aligns with human perception~\cite{zhang2018Lpips}, deep neural networks are also well known to be biased towards certain attributes, such as texture~\cite{geirhos2018CnnBiasTexture} and background~\cite{sehwag2020BackgroundCheck, xiao2021NoiseorSignal}. Our sampling process can exploit these biases, such as by simply removing the background, to induce a large change in the likelihood in feature space. We also conduct an examination to investigate signs of memorization and whether our sampling process is exploiting them. While we didn't observe any memorization on the ImageNet dataset, diffusion models might memorize samples on even more complex and non-curated datasets than ImageNet. In event of such memorization, our sampling process might exploit it. 

% Our work provides the unique capability of sampling novel yet rare to occur samples from data distributions. 

Deep neural networks often struggle to generalize to novel and rarely observed samples from the distribution~\cite{hendrycks2021naturalAdv, koh2021WILDS}. We believe that our work can further assist in improving the distributional robustness of these networks. Our sampling process also reveals that diffusion models successfully generalize to low-density regions of data manifold which further strengthens the argument that these models hold the potential to provide tremendous benefits in representation learning~\cite{sehwag2021ProxyDist, gowal2021GeneratedData}.   



% For example, it is well known that the \textit{tench fish class} images in ImageNet often include a human holding the fish. Supervised classifier picks up this bias and learns to correlate the output with the human in the background. We often observe that the generative model simply removes the human from the background, thus incurring a large effect on its embeddings due to the bias of the classifier.

==> Diverse sampling from generative models [CVPR 22]/sections_old/application.tex <==
\subsection{Comprehensive evaluation of discriminative models}
\dummytext{2}

\noindent \textbf{Filtering low-fidelity images using an Oracle.} While we do optimize to fidelity when increasing hard instances, the generative model might still provide some model low-fidelity or not photorealistic samples. As such samples are out-of-distribution, the first steps is to filter these out. However, it is very challenging since it requires distinguishing these out-of-distribution instances from hard instances (show examples of both). Simply using a classifier output is not enough, as it leads to a poor classification prediction on both. So how do we construct of good Oracle ($\gF$). Of course, a human in loop is the ideal approach, as it is done for collecting many other real-world datasets. However, it is not scalable. So the next question is how to develop a automated but a good Oracle.




\textit{Evaluating the quality of an Oracle.} We measure the quality of an Oracle by its success in recognizing hard to learn but high fidelity real-world examples while discarding out-of-distribution data. 

We provide a detailed description of our approach in Appendix xyz. 

We can also finetune a particular classifier (or train on jointly) on the hard instances. This will show that these instances are indeed learnable (thus aren't garbage) and current models don't end of learning them. 

We need a way to calibrate the scale of this oracle. May calibrate from real-dataset such as ObjectNet, ImageNet-C etc. Or we can ourselves heavily deteriorate images to gather a better insight into this threshold. 

==> Diverse sampling from generative models [CVPR 22]/sections_old/discussion.tex <==
While synthetic data is known to improve learning in biomedical domains~\citep{chen2021syntheticBioML}, this is not yet true for complex datasets like ImageNet. Still do happen for CIFAR-10. This could be the focus of future research work.

Comments from \textit{Michal Drozdzal}: 1) Two different long-tailed challenges - a) in images (hard vs easy) b) in classes (highly vs poorly represented classes). We tackle the former not latter. 2) Data augmentation is one key factor we can use to obtain even a better set of models (this would be another building block in my idea of using better oracles/feature-extractor for this).

\textbf{What about memorization.} Generative language models are known to memorize low-density hard instances. Is low-density sampling from our model simply generating memorized instances?

\textbf{Minimizing hardness.} There our methods becomes similar to OPENAI's work. But does the different loss function, loss normalization etc. lead to a different FID score? Make sure to use a clean-fid implementation. 


==> Diverse sampling from generative models [CVPR 22]/sections_old/introduction.tex <==
\subsection{Outline}
\begin{itemize}
    \item Introduction (~2 pages)
    \item On sampling hard instance from diffusion models 
    \begin{itemize}
        \item Overview of working and sampling from diffusion models (2.5 pages)
        \item Motivation of hard instance sampling and limitation of existing approach (3)
        \item Our framework (~4 pages)
        \item Empirical validation of each control block in the framework (~5 pages)
    \end{itemize}
    \item Applications
    \begin{itemize}
        \item Comprehensive evaluation of existing models. We evaluated pre-trained model over different hardness scales. (6 pages)
        \item Improving robustness when combining with real data. (7 pages) 
    \end{itemize}
\end{itemize}

\dummytext{4}

\subsection{Key contributions}
\begin{itemize}
    \item We characterize the spread of distribution of images generated by common generative models and highlight how diffusion based models generate harder instances i.e., data is spread across the hardness scale. \vikash{Use real images from validation set. Ablations with different feature extractor and distance metrics in appendix.}
    \item We further demonstrate that diffusion based models can generate even harder instances. We achieve so by using simultaneously optimizing for hardness when solving diffusion process. 
    \item We use this ability to control hardness to provide a comprehensive evaluation of robustness of pre-trained models to distribution shift. In particular, we show that accuracy of pre-trained models degrades significantly as we move to low density regions on the training distribution. 
    \item Optimistically, using synthetic-sample from low-density regions will improve the performance on these hard instances from low-density regions.
    \item So far we only measure generalization on synthetic data. What about synthetic to real generalization. We find that training on hard-instances can further improve generalization to large distribution shifts. \vikash{On ImageNet, combining synthetic and real dataset hurts performance rather than improving it. We aren't there yet on ImageNet, but we can use some other small scale dataset to show these results.}
\end{itemize}


\subsection{Additional comments}

Potential downstream benefits of using synthetic data beyond improving accuracy. If most of them are successful, this can go into a separate paper on its own. 
\begin{itemize}
    \item \textbf{Robustness.} Check out robustness to standard benchmarks, such as ImageNet-C, ImageNet-R etc.
    \item \textbf{Faster convergence}. Using additional data make it converge faster. However, its true only when we don't count extra synthetic data in each batch i.e., now we are training on double the amount of images. 
    \item \textbf{Better calibration.} We can also check whether confidence values are more calibrated with synthetic data. Also whether out-of-distribution detection and privacy leakage are also reduced. 
\end{itemize}


Few things we can do to provide deeper insights:
\begin{itemize}
    \item Check effect on fine-grained vs coarse-grained classification. It likely that generative models will struggle with the fine-grained classification aspect i.e., improvement in hard classes (such as breeds of dogs) will be lower than other random classes. 
    \item Synthetic data as data-augmentation when combined with real data. This is another perspective to discuss results with synthetic data. 
    \item Check effect of synthetic data on a diverse range of networks. It might be most beneficial for low capacity network, such as Mobilenet etc. 
\end{itemize}


==> Diverse sampling from generative models [CVPR 22]/sections_old/methods.tex <==
\dummytext{2}

\subsection{How to measure hardness of a test instance?}
This is the metric we will use to measure how hard/diverse/from-tail-of-distribution this sample is. It will mostly be use for evaluation purposed. We will provide its comparison with other evaluation metrics in the appendix (also connect to existing evaluation metrics known for GANs). \dummytext{2}

We argue that probability density of the distribution can be used to measure hardness. In particular, we samples in low-density regions will be less representative in training data, thus likely be hard to learn. The key design choice is how to estimate the probability density of each sample. Since the underlying data distribution is unknown, we estimate the probability by modelling each class samples using a Gaussian distribution. To achieve a better estimate we model features extracted from a pre-trained classifier. We present detailed results and discussion on choice of feature extractor and modelling distributions in Appendix xyz. \vikash{Even all white/black image are near tail of distribution, it doesn't mean they hard to learn.}

\textbf{Choice of feature extractor.} To reliably estimate hardness of low probability samples, we need a model that provide correct representation of low density samples. However, when real dataset itself has a long-tailed probability distribution, most classifiers often lead to incorrect prediction on low-density samples. This generalization to hard real instances in commonly measured by generalization to ImageNet-A, which is a collection of $7.5$K images (cite timm). We use the top-ranking models on this dataset as feature extractor. Top-ranking models achieve better generalization to low-density regions by using extra training data along with highly expressive deep neural networks.

\textit{Why not use output softmax probabilities.} They are simply not calibrated as almost all images have very high confidence. Similarly existing metrics like likelihood score, FID, precision-recall are not samples specific, thus not suitable for our task. 

\textbf{Instance hardness} We define instances are hardness using the probability of given sample. In particular we measure it using the negative log-prob from normal distribution over embeddings. Lower the probability of given instance, harder it is. 

\begin{figure}
    \centering
    \includegraphics{images/hardness_score_comparison_generative_model.pdf}
    \caption{\textbf{Why use diffusion-based models?} Comparison of hardness scores of synthetic images generated using uniform sampling from the DDPM and BigGAN models. Unlike BigGAN, which generates highly photorealistic but easier instances, diffusion based model is able to generate much harder instances. However, note that uniform sampling leads to a long-tail distribution, i.e., it samples more instances from low-density (easier) regions.}
    \label{fig:my_label}
\end{figure}


\subsection{Which generative model to use? or Why use diffusion models?}
We use score-based generative models. Multiple reasons for this 1) They simple outperform GANs at sample quality 2) They can provably learn all modes of data. Second factor is most crucial to us since we need a model that has truly learned the data distribution. If its only learning a few directions (boundary collapse), then it won't capture the whole distribution, thus we can't sample any hard instance form it. We can provide a quantitative comparison of hardness of samples generated from diffusion models and GANs and compare them to real world. Likely without any tricks, diffusion models will provide better (even match) the hardness of real world samples. 


\subsection{Proposed framework to improve hardness of synthetic samples}

% \begin{figure}
%     \centering
%     \includegraphics{images/instance_hardness_score_with_temp_0.1_euclidean_softmax.pdf}
%     \caption{\textbf{Controlling hardness of generate instances?} By changing the scaling parameter, we show that hardness of generated instances can be controlled. \vikash{Add a few example images at major hardness score values.}}
%     % \label{fig:my_label}
% \end{figure}


\subsection{Outline}
\begin{itemize}
    \item With the goal of enabling sampling from low-density regions, we use additional gradient step from a classifier. We start with the softmax probabilities, which are a common choice to optimize, though mostly for improving image fidelity. We are the first one to show that they can be used to move to low-density region. A common challenge with softmax probs is that even OOD data can have high probabilities. To get a precise measure of distance from existing images we work in the feature space.
    We provide a detailed analysis on success and limitation of each loss function. 
    \begin{itemize}
            \item We have yet to explore batch-wise loss functions.
    \end{itemize}
    \item Again no single scale value is precise, as some generated samples are out of distribution or not visually realistic. But for simiplicty lets just fix one scale. Even there we want to choose images (for evaluation or training) that are hard yet have high fidelity. One example where this is needed is when we combine synthetic data with real. Even uniformly sampled images, which are of high fidelity, hurt performance, rather than improving it.
    \begin{itemize}
        \item One question that will come up is why we don't optimize for it. Answer could be that to incorporate it in ddpm pipeline, we need to make an noise invariant approach, which naturally makes it harder. 
    \end{itemize}
    \begin{itemize}
            \item This question is hard to answer than a similar question in active learning (https://dsgissin.github.io/DiscriminativeActiveLearning/2018/07/05/AL-Intro.html) since we even a out-of-distribution data which can have high entropy but doesn't belong to the distribution. 
    \end{itemize}
    \item A unique approach to testing images at difference hardness scales. Once we fix hyperparameters for all factors, we can start tuning the hardness parameters and measure the accuracy of the classifier at each hardness scale. If we can assure that visual semantics are intact, \textit{this could be one evidence of how existing classifier fails near the tail of the distribution.} Pitch this as some sort of more rigorous or in-depth evaluation of models. Test all state-of-the-art models.
    \begin{itemize}
            \item See if we can filter out garbage/outlier images from the image that are truly hard to learn but have correct semantics. May be bring a human in the loop.
            \item ToDo: Construct a set of ~100-500K images at each hardness scale for ImageNet. Next filter out the ones with highest fidelity (using human in the loop) or reject the ones with lowest. May be ask folks to throw images in one of the three columns 1) high fidelity 2) Moderate fidelity 3) Poor fidelity. 
    \end{itemize}
\end{itemize}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_992.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_323.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_985.jpeg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_130.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_89.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_604.jpeg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_900.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_779.jpeg}
    \end{subfigure}
    \caption{Demo hardness with sample images. Cite common semantic variations such as viewpoint, color in flowers, background (bus is sky) etc.}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/hardness_score_comparison_across_all_scales.pdf}
    \caption{Experimentally validating that tuning hardness scales does shift the resulted hardness score of images.}
\end{figure}

\begin{table}[]
    \centering
    \caption{Comparing the sample generation time of our method (scale=1.0) with uniform sampling. Each entry represents the time taken to generate $50$K $256\times256$ resolution synthetic images from the corresponding score range.}
    \begin{tabular}{cccc}  \toprule
     Score-range & $100-120$ & $120-140$ & $140-160$ \\ \midrule
     \base & $19.9$ & $57.4$ & $167.9$ \\ 
     \ours & $18.8$ \scriptsize{($\times \textbf{1.1}$)}  & $20.3$ \scriptsize{($\times \textbf{2.8}$)} & $27.8$ \scriptsize{($\times \textbf{6.0}$)} \\ \bottomrule
     % [18.1 20.4 29.4] (scale=0.5), [17.2 28.  50.6] (scale=0.1), [16.9 23.6 37.3](scale=0.2), [18.  36.4 75.7](scale=0.05), [ 24.   67.7 187.2](scale=0.005)
    \end{tabular}
\end{table}


\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_992.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_323.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_985.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_130.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_89.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_604.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_900.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_779.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_0.jpeg}
    \end{subfigure}
    \caption{Progressive hardening of samples. TODO: Also display hardness score below each image.}
\end{figure}


\begin{figure}
    \centering
    \includegraphics{images/per_class_accuracy_baseline_synthetic.pdf}
    \caption{Top-1 per-class accuracy for synthetic data. We threshold the classes as the mean accuracy over real imagenet validation images, i.e., 77.6. Highlight ImageNet-400 in plot itself.}
\end{figure}



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet400_top1.pdf}
        \caption{ImageNet-400 (top-1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet400_top5.pdf}
        \caption{ImageNet-400 (top-5)}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet_top1.pdf}
        \caption{ImageNet (top-1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet_top5.pdf}
        \caption{ImageNet (top-5)}
    \end{subfigure}
    \caption{Comprehensive evaluation of existing pre-trained models with increasing hardness score. To avoid statistical noise, we plot accuracy for each score range only when at least 5 images for each class are available. Given limited number of samples in real data, its not feasible to do a accurate evaluation of robustness over all score values. TODO: just for the sake of it, also provide full real-data curves in appendix.}
\end{figure}


\begin{table}[!htb]
    \centering
    \caption{Top-1 accuracy on original \textit{ImageNet-400} dataset and some of its domain shifted versions. (R) refers to using only real data where (R+S) refers to using real and synthetic data together in training. TODO: Also provide top-5 accuracy results.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc|cc} \toprule
        Architecture & Data & Original & ImageNet-Rendition & ImageNet-sketch  \\ \midrule
        \multirow{3}{*}{ResNet-18} & R & $88.4$ &  $28.9$ & $28.5$ \\
         & R + S (uniform) & $88.7$ \scriptsize{($\textbf{+0.3}$)} &  $29.5$ \scriptsize{($\textbf{+0.6}$)} & $31.1$ \scriptsize{($\textbf{+2.6}$)}  \\
         & R + S (\ours) & $88.3$ \scriptsize{($\textbf{-0.3}$)} &  $30.2$ \scriptsize{($\textbf{+1.3}$)} & $32.2$ \scriptsize{($\textbf{+3.7}$)} \\ \midrule
        \multirow{3}{*}{ResNet-50} & R & $91.6$ &  $32.5$ & $30.0$ \\
         & R + S (uniform) & $91.5$ \scriptsize{($\textbf{-0.1}$)} &  $33.4$ \scriptsize{($\textbf{+0.9}$)} & $34.3$ \scriptsize{($\textbf{+4.3}$)} \\
         & R + S (\ours) & $91.4$ \scriptsize{($\textbf{-0.2}$)} &  $33.9$ \scriptsize{($\textbf{+1.4}$)} & $35.4$ \scriptsize{($\textbf{+5.4}$)} \\ \midrule
        \multirow{3}{*}{ResNet-101} & Real & $92.4$ &  $34.7$ & $35.7$ \\
         & R + S (uniform) & $92.3$ \scriptsize{($\textbf{-0.1}$)} &  $36.1$ \scriptsize{($\textbf{+1.4}$)} & $38.7$ \scriptsize{($\textbf{+3.0}$)} \\
         & R + S (\ours) & $92.2$ \scriptsize{($\textbf{-0.2}$)} &  $36.2$ \scriptsize{($\textbf{+1.5}$)} & $38.6$ \scriptsize{($\textbf{+2.9}$)}  \\ \bottomrule
    \end{tabular}}
\end{table}

\begin{table}[!htb]
    \centering
    \caption{Top-1 accuracy on original full \textit{ImageNet-1K} dataset and some of its domain shifted versions. (R) refers to using only real data where (R+S) refers to using real and synthetic data together in training.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc|cc} \toprule
        Architecture & Data & Original & ImageNet-Rendition & ImageNet-sketch  \\ \midrule
        \multirow{3}{*}{ResNet-18} & R & $70.6$ &  $22.4$ & $23.0$ \\
         & R + S (uniform) & $70.2$ \scriptsize{($\textbf{-0.4}$)} &  $22.2$ \scriptsize{($\textbf{-0.2}$)} & $22.8$ \scriptsize{($\textbf{-0.2}$)}  \\
         & R + S (\ours) & $69.3$ \scriptsize{($\textbf{-1.3}$)} &  $22.2$ \scriptsize{($\textbf{-0.2}$)} & $22.6$ \scriptsize{($\textbf{-0.4}$)} \\ \midrule
        \multirow{3}{*}{ResNet-50} & R & $77.6$ &  $26.9$ & $27.4$ \\
         & R + S (uniform) & $77.2$ \scriptsize{($\textbf{-0.4}$)} &  $27.3$ \scriptsize{($\textbf{+0.4}$)} & $28.9$ \scriptsize{($\textbf{+1.5}$)} \\
         & R + S (\ours) & $77.1$ \scriptsize{($\textbf{-0.5}$)} &  $27.3$ \scriptsize{($\textbf{+0.4}$)} & $28.6$ \scriptsize{($\textbf{+1.2}$)} \\ \midrule
        \multirow{3}{*}{ResNet-101} & Real & $--$ &  $--$ & $--$ \\
         & R + S (\ours) & $--$ &  $--$ & $--$  \\ \bottomrule
    \end{tabular}}
\end{table}

==> sections/applications.tex <==
% Two ways to compare results. 
% 1. Uniforms vs synthetic ours: How much does distribution coverage benefits us. May be not too much as we don't have much samples in high density regions, which real data expects. May be see if we stable more on robustness. 
% Plot the final hardness score of both ours and baseline to give some context there.
% 2. 



==> sections/rel_work.tex <==
We discuss papers from each related domains to ours. Since we already devote a significant space to background of diffusion models in methods, its not wise to put related work at the start. Otherwise it will be already 3-4 pages before the reader arrives at our core contributions. Anyway we aren't advancing our previous work, since this work is pretty tangential to most previous paper in generative modelling. 

\noindent \textbf{Diffusion based generative models.} This includes details on diffusion models. Few lines of how they are better than other generative models. \dummytext{4}

\noindent \textbf{Sampling techniques from generative models.} 
Discuss top-k sampling in VAE papers, Bean search and nucleus sampling in language models (GPT papers).
\dummytext{6}

\noindent \textbf{Synthetic-to-real domain transfer.} \dummytext{5}

\noindent \textbf{Robustness to domain-shifts.} \dummytext{6}

\noindent \textbf{Miscellaneous.} \dummytext{2}


\section{Further discussion}
\begin{itemize}
    \item There have been previous work on GANs on diverse sampling. Since all of us just uses a fixed generative model but modifies the procedure, it matter how good is generative model. As we show, ddpm models are better than gans, thus making our work of prime importance. But lets also make sure that it doesn't look like that we are doing an incremental work (since ddpm model has very novel challenge than gans). Lets discuss this previous work early on (like whats hiding in our networks paper).
    \item When comparing timing cost, also compare with cost when using fast sampling criterion. But argue that our techniques can be used with fast samplers too. 
    \item Lets focus on insights, even before jumping to applications. What hidden in the generative model?  If the data manifold modelled well for all classes.  I mean can it generate hard images well for all classes? If not then why not?
    \item Fig. 1 is main pitch. Put biggan, ddpm, and ours images. GANs can't do much due to poor coverage. DDPM model is much better (as we will also show) and we improve its ability a lot. 
    \item How about we also incorporate these images in our framework on proxy distributions. The might further boost the performance of adversarial training. 
    \item We might also need to retrain the diffusion models for some ablation studies, i.e., why did the diffusion network modelled low-density manifold so well? Will even limited number of samples from these regions make it worse?
    \item In memorization, do a very water tight analysis. Calculate pairwise distance (with 1M synthetic and 1M real images) and flag images that are super close to each other. 
    \item Are these examples adversarial? No, as slight variation in objective leads to perceptible changes, not adversarial ones.. Even if there are some, we choose to use a different network in our analysis (resnet50) than one used in optimization.
    \item How about we use a toy experiment like using mixture-of-Gaussian to explain our idea a bit more intuitively (something like \url{https://openreview.net/pdf?id=lsQCDXjOl3k}).
    \item Compare with VQGAN too when arguing about use of diffusion based models. BigGAN comparison just seems to naive and will invite further criticism.
    \item Before applications, add another section on analyzing low-density samples. We analyze 1) if the network is simply memorizing them 2) the intriguing transformation network exploit to generate them 3) Some likelihood to verify that they are low-density (don't use classifier to do it)
    \item Arange related work in 1) Selective sampling (Discriminator Rejection Sampling, VAE and many others for high fidelity, LOGAN and other for high diversity). 2) Benefit of synthetic data (in benign and adversarial training). Ideally humans are best for rejecting/accpeting samples (as argued in future work of discriminator rejection sampling paper).
    \item Why don't we also use a discriminator (like discriminator rejection sampling) to make sure that we stay close to the real data distribution. Say random sampling lead to true distribution but higher $\alpha$ led to much different distribution. We might have moved too far from real-data distribution then. We need to ensure that it doesn't happen. This could serve as an visualization of our approach. 
    \item Use concrete terms like top-k sampling, nucleus sampling and provide comparison with them.
    \item We also uncovered that some classes for the dataset have much less coverage of the distribution that others, since the fidelity of images quickly degraded.
    \item Compare with other related papers that are under submission at ICLR. 
    \item Its not hard instances that we are after. True our framework can generate both easy and hard instances. Hard instances is also a vague term. What we specifically are optimizing for is to generate rate to occur samples from training data. Even more samples that are absent from training data, but somehow the generate model construct them out of nowhere. 
    \item To motivate the problem, we can first show both high and low-likelihood images in training set. GAN are known to not model low-likelihood. Diffusion model seems to do it but random sampling doesn't suffice. We develop techniques to sample low-likelihood images from diffusion based models. So spli figure 1, real images into two. Keep some space between Real and others.
    \item Generate some 512x512 images for visualization.
    \item Again Hardness is very subjective metric. Lets tick to using likelihood as a measure of whether the sample belong to low-density region of the distribution.
    \item Goal to meet: You must make your paper easy to read. You've got to make it easy for anyone to tell what your paper is about, what problem it solves, why the problem is interesting, what is really new in your paper (and what isn't), why it's so neat.
    \item How training on low density data helps. How about we train on synthetic (random vs ours) and test on real (training set since test set doesn't have enough images). There can our approach slow down the rate at which accuracy degrades (even if it start at a smaller accuracy for easier images). 
    \item To constructively demonstrate the impact of both loss terms, lets display a grid. Starting from one image, change one coefficient on one axis and another coefficient. Do it for 3-5 images, keep one in the main paper and rest in the appendix.
    \item Lets try to follow a similar presentation style as original StyleGAN paper: https://arxiv.org/pdf/1812.04948.pdf
    \item To compare with random sampling (in training aspect), we can use a use a dataset which is unformly distributed, unlike a long-tail distribution like real data or random sampling. 
    \item Motivation in methods section. Mention that in low-density regions, not much samples are available, thus the generative distribution may lie far away from real data distribution. Its most critical that we use a guidance term there. It will become evident from our plot that this additional loss term has most impact when the distance from the centroid of the manifold is highest.
    \item Lets stick to only a few things in the analysis: Memorization and class-wise discrepancy and that's all. Too much content leads to much high exposure.
    \item A baseline for us could be the Nyguen paper on BigGAN diverse sampling or LoGAN. Both are both GANs, which are totally different from Diffusion models. Nevertheless, we try the class-condition smoothing idea but find that diffusion model doesn't respond very well and quickly generates poor quality images. In contrast our approach work very well. 
    \item Put the results on OOD robustness in the appendix of the paper (since we don't have a conclusive trend there). 
    \item We argue that for low-density sample the model quickly generated bad samples. What would be analogy in terms of scores. Are score in low-density region not define well (due to lack of data) and thus not learned well.
    \item By default the model is trained to maximize the likelihood (or lower bound) at each transition. Our approach allows us to guide model toward low-likelihood, but still on-manifold regions. \item Though we are first to try this idea on ddpm, lets compare with a few baselines on ddpm itself: 1) with class smoothing 2) optimizing on x-start instead of x-t in the diffusion process. 
    \item Note that our samples are continuous in the diffusion process, so we can't talk about their point probabilities (only true for x-start which is discrete). Also likelihood core definition that it is regarded as the likelihood of a set of parameters give outcomes. So its more natural to talk about likelihood when optimizing parameters (since its parameters likelihood that we are optimizing, give observed values). But it doesn't make sense to talk about instance likelihood. 
    \item How do we argue that the model is biased to sample from high-density region, as more data is centered there. 
    \item Contrast out approach with interpolation in low-density space, i.e., from where no novel images are seen at training time, such as work on Dall-E.
    \item Lets also add a section where we compare the density of generated samples using other distance metrics, such as k-nn, likelihood, changing representation spaces etc.  
    \item Discuss Vitaly Feldman's paper on long tale, which argues the its necessary to memorize low-density data otherwise the network may not generalize there. 
    \item Make sure to include coverage of distribution from multiple other metrics, such as recall, k-nn neighbors etc. 
    \item To address limitation of our method to supervised setting, also add another section of using contrastive learning based loss for unsupervised setting (assuming a supervised classifier is available). 
    \item Contrast to ML paper, follow style of a common CVPR paper: \url{http://selfcondgan.csail.mit.edu/preprint.pdf}. Similar to their fig. 4, add visual examples comparing our approach with uniform sampling and real images. 
    \item In appendix add a comparison section of different likelihood esitmation metric. Take 20 images from an easy class from ImageNet and sort them based on each of the metric. See which metric do well and which don't. May be add some basic negative too (like white noise, all-black pixel images etc to test the robustness). We can refer to this plot to justify why we didn't optimize the model likelihood and why we choose the embedding space to optimize.
    \item To justify why higher alpha makes things worse since model distribution is not accurate, plot the results with minimizing negative log-likelihood and show that there the model can sustain much higher values of alpha but not in the other direction.
    \item Address the selective vs random picking of visual examples. 
    \item Use visualization with the images generated from the embedding loss, instead of soft-max loss (even though they are mostly equivalent). 
    \item One might ask, how high is the fidelity of our generated samples? Well that's hard to answer, since existing generative models have trouble generalizing to them.
    \item Can we also show that our work can be further integrated with ddim and other fast sampling approaches?
    \item Make sure to include demo images from CIFAR-10 dataset too, otherwise we will be shot-down for just using one dataset.
    \item Discuss the instability in the inverse of covariance matrix at higher time stamps. We need to talk about it in the experimental setup section or the methods itself. Note that this is only the case for optimization. As inference, when t=0, we do consider sigma without any approximation. 
    \item We also need to discuss the selection procedure for alpha and beta, in particular when selecting images for some applications.
    \item 
\end{itemize}
% Why we don't end up generating adversarial examples.


==> sections_old/application.tex <==
\subsection{Comprehensive evaluation of discriminative models}
\dummytext{2}

\noindent \textbf{Filtering low-fidelity images using an Oracle.} While we do optimize to fidelity when increasing hard instances, the generative model might still provide some model low-fidelity or not photorealistic samples. As such samples are out-of-distribution, the first steps is to filter these out. However, it is very challenging since it requires distinguishing these out-of-distribution instances from hard instances (show examples of both). Simply using a classifier output is not enough, as it leads to a poor classification prediction on both. So how do we construct of good Oracle ($\gF$). Of course, a human in loop is the ideal approach, as it is done for collecting many other real-world datasets. However, it is not scalable. So the next question is how to develop a automated but a good Oracle.




\textit{Evaluating the quality of an Oracle.} We measure the quality of an Oracle by its success in recognizing hard to learn but high fidelity real-world examples while discarding out-of-distribution data. 

We provide a detailed description of our approach in Appendix xyz. 

We can also finetune a particular classifier (or train on jointly) on the hard instances. This will show that these instances are indeed learnable (thus aren't garbage) and current models don't end of learning them. 

We need a way to calibrate the scale of this oracle. May calibrate from real-dataset such as ObjectNet, ImageNet-C etc. Or we can ourselves heavily deteriorate images to gather a better insight into this threshold. 

==> sections_old/discussion.tex <==
While synthetic data is known to improve learning in biomedical domains~\citep{chen2021syntheticBioML}, this is not yet true for complex datasets like ImageNet. Still do happen for CIFAR-10. This could be the focus of future research work.

Comments from \textit{Michal Drozdzal}: 1) Two different long-tailed challenges - a) in images (hard vs easy) b) in classes (highly vs poorly represented classes). We tackle the former not latter. 2) Data augmentation is one key factor we can use to obtain even a better set of models (this would be another building block in my idea of using better oracles/feature-extractor for this).

\textbf{What about memorization.} Generative language models are known to memorize low-density hard instances. Is low-density sampling from our model simply generating memorized instances?

\textbf{Minimizing hardness.} There our methods becomes similar to OPENAI's work. But does the different loss function, loss normalization etc. lead to a different FID score? Make sure to use a clean-fid implementation. 


==> sections_old/introduction.tex <==
\subsection{Outline}
\begin{itemize}
    \item Introduction (~2 pages)
    \item On sampling hard instance from diffusion models 
    \begin{itemize}
        \item Overview of working and sampling from diffusion models (2.5 pages)
        \item Motivation of hard instance sampling and limitation of existing approach (3)
        \item Our framework (~4 pages)
        \item Empirical validation of each control block in the framework (~5 pages)
    \end{itemize}
    \item Applications
    \begin{itemize}
        \item Comprehensive evaluation of existing models. We evaluated pre-trained model over different hardness scales. (6 pages)
        \item Improving robustness when combining with real data. (7 pages) 
    \end{itemize}
\end{itemize}

\dummytext{4}

\subsection{Key contributions}
\begin{itemize}
    \item We characterize the spread of distribution of images generated by common generative models and highlight how diffusion based models generate harder instances i.e., data is spread across the hardness scale. \vikash{Use real images from validation set. Ablations with different feature extractor and distance metrics in appendix.}
    \item We further demonstrate that diffusion based models can generate even harder instances. We achieve so by using simultaneously optimizing for hardness when solving diffusion process. 
    \item We use this ability to control hardness to provide a comprehensive evaluation of robustness of pre-trained models to distribution shift. In particular, we show that accuracy of pre-trained models degrades significantly as we move to low density regions on the training distribution. 
    \item Optimistically, using synthetic-sample from low-density regions will improve the performance on these hard instances from low-density regions.
    \item So far we only measure generalization on synthetic data. What about synthetic to real generalization. We find that training on hard-instances can further improve generalization to large distribution shifts. \vikash{On ImageNet, combining synthetic and real dataset hurts performance rather than improving it. We aren't there yet on ImageNet, but we can use some other small scale dataset to show these results.}
\end{itemize}


\subsection{Additional comments}

Potential downstream benefits of using synthetic data beyond improving accuracy. If most of them are successful, this can go into a separate paper on its own. 
\begin{itemize}
    \item \textbf{Robustness.} Check out robustness to standard benchmarks, such as ImageNet-C, ImageNet-R etc.
    \item \textbf{Faster convergence}. Using additional data make it converge faster. However, its true only when we don't count extra synthetic data in each batch i.e., now we are training on double the amount of images. 
    \item \textbf{Better calibration.} We can also check whether confidence values are more calibrated with synthetic data. Also whether out-of-distribution detection and privacy leakage are also reduced. 
\end{itemize}


Few things we can do to provide deeper insights:
\begin{itemize}
    \item Check effect on fine-grained vs coarse-grained classification. It likely that generative models will struggle with the fine-grained classification aspect i.e., improvement in hard classes (such as breeds of dogs) will be lower than other random classes. 
    \item Synthetic data as data-augmentation when combined with real data. This is another perspective to discuss results with synthetic data. 
    \item Check effect of synthetic data on a diverse range of networks. It might be most beneficial for low capacity network, such as Mobilenet etc. 
\end{itemize}


==> sections_old/methods.tex <==
\dummytext{2}

\subsection{How to measure hardness of a test instance?}
This is the metric we will use to measure how hard/diverse/from-tail-of-distribution this sample is. It will mostly be use for evaluation purposed. We will provide its comparison with other evaluation metrics in the appendix (also connect to existing evaluation metrics known for GANs). \dummytext{2}

We argue that probability density of the distribution can be used to measure hardness. In particular, we samples in low-density regions will be less representative in training data, thus likely be hard to learn. The key design choice is how to estimate the probability density of each sample. Since the underlying data distribution is unknown, we estimate the probability by modelling each class samples using a Gaussian distribution. To achieve a better estimate we model features extracted from a pre-trained classifier. We present detailed results and discussion on choice of feature extractor and modelling distributions in Appendix xyz. \vikash{Even all white/black image are near tail of distribution, it doesn't mean they hard to learn.}

\textbf{Choice of feature extractor.} To reliably estimate hardness of low probability samples, we need a model that provide correct representation of low density samples. However, when real dataset itself has a long-tailed probability distribution, most classifiers often lead to incorrect prediction on low-density samples. This generalization to hard real instances in commonly measured by generalization to ImageNet-A, which is a collection of $7.5$K images (cite timm). We use the top-ranking models on this dataset as feature extractor. Top-ranking models achieve better generalization to low-density regions by using extra training data along with highly expressive deep neural networks.

\textit{Why not use output softmax probabilities.} They are simply not calibrated as almost all images have very high confidence. Similarly existing metrics like likelihood score, FID, precision-recall are not samples specific, thus not suitable for our task. 

\textbf{Instance hardness} We define instances are hardness using the probability of given sample. In particular we measure it using the negative log-prob from normal distribution over embeddings. Lower the probability of given instance, harder it is. 

\begin{figure}
    \centering
    \includegraphics{images/hardness_score_comparison_generative_model.pdf}
    \caption{\textbf{Why use diffusion-based models?} Comparison of hardness scores of synthetic images generated using uniform sampling from the DDPM and BigGAN models. Unlike BigGAN, which generates highly photorealistic but easier instances, diffusion based model is able to generate much harder instances. However, note that uniform sampling leads to a long-tail distribution, i.e., it samples more instances from low-density (easier) regions.}
    \label{fig:my_label}
\end{figure}


\subsection{Which generative model to use? or Why use diffusion models?}
We use score-based generative models. Multiple reasons for this 1) They simple outperform GANs at sample quality 2) They can provably learn all modes of data. Second factor is most crucial to us since we need a model that has truly learned the data distribution. If its only learning a few directions (boundary collapse), then it won't capture the whole distribution, thus we can't sample any hard instance form it. We can provide a quantitative comparison of hardness of samples generated from diffusion models and GANs and compare them to real world. Likely without any tricks, diffusion models will provide better (even match) the hardness of real world samples. 


\subsection{Proposed framework to improve hardness of synthetic samples}

% \begin{figure}
%     \centering
%     \includegraphics{images/instance_hardness_score_with_temp_0.1_euclidean_softmax.pdf}
%     \caption{\textbf{Controlling hardness of generate instances?} By changing the scaling parameter, we show that hardness of generated instances can be controlled. \vikash{Add a few example images at major hardness score values.}}
%     % \label{fig:my_label}
% \end{figure}


\subsection{Outline}
\begin{itemize}
    \item With the goal of enabling sampling from low-density regions, we use additional gradient step from a classifier. We start with the softmax probabilities, which are a common choice to optimize, though mostly for improving image fidelity. We are the first one to show that they can be used to move to low-density region. A common challenge with softmax probs is that even OOD data can have high probabilities. To get a precise measure of distance from existing images we work in the feature space.
    We provide a detailed analysis on success and limitation of each loss function. 
    \begin{itemize}
            \item We have yet to explore batch-wise loss functions.
    \end{itemize}
    \item Again no single scale value is precise, as some generated samples are out of distribution or not visually realistic. But for simiplicty lets just fix one scale. Even there we want to choose images (for evaluation or training) that are hard yet have high fidelity. One example where this is needed is when we combine synthetic data with real. Even uniformly sampled images, which are of high fidelity, hurt performance, rather than improving it.
    \begin{itemize}
        \item One question that will come up is why we don't optimize for it. Answer could be that to incorporate it in ddpm pipeline, we need to make an noise invariant approach, which naturally makes it harder. 
    \end{itemize}
    \begin{itemize}
            \item This question is hard to answer than a similar question in active learning (https://dsgissin.github.io/DiscriminativeActiveLearning/2018/07/05/AL-Intro.html) since we even a out-of-distribution data which can have high entropy but doesn't belong to the distribution. 
    \end{itemize}
    \item A unique approach to testing images at difference hardness scales. Once we fix hyperparameters for all factors, we can start tuning the hardness parameters and measure the accuracy of the classifier at each hardness scale. If we can assure that visual semantics are intact, \textit{this could be one evidence of how existing classifier fails near the tail of the distribution.} Pitch this as some sort of more rigorous or in-depth evaluation of models. Test all state-of-the-art models.
    \begin{itemize}
            \item See if we can filter out garbage/outlier images from the image that are truly hard to learn but have correct semantics. May be bring a human in the loop.
            \item ToDo: Construct a set of ~100-500K images at each hardness scale for ImageNet. Next filter out the ones with highest fidelity (using human in the loop) or reject the ones with lowest. May be ask folks to throw images in one of the three columns 1) high fidelity 2) Moderate fidelity 3) Poor fidelity. 
    \end{itemize}
\end{itemize}

\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_992.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_323.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_985.jpeg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_130.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_89.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_604.jpeg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_900.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_hardness_interpolate_samples_class_779.jpeg}
    \end{subfigure}
    \caption{Demo hardness with sample images. Cite common semantic variations such as viewpoint, color in flowers, background (bus is sky) etc.}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/hardness_score_comparison_across_all_scales.pdf}
    \caption{Experimentally validating that tuning hardness scales does shift the resulted hardness score of images.}
\end{figure}

\begin{table}[]
    \centering
    \caption{Comparing the sample generation time of our method (scale=1.0) with uniform sampling. Each entry represents the time taken to generate $50$K $256\times256$ resolution synthetic images from the corresponding score range.}
    \begin{tabular}{cccc}  \toprule
     Score-range & $100-120$ & $120-140$ & $140-160$ \\ \midrule
     \base & $19.9$ & $57.4$ & $167.9$ \\ 
     \ours & $18.8$ \scriptsize{($\times \textbf{1.1}$)}  & $20.3$ \scriptsize{($\times \textbf{2.8}$)} & $27.8$ \scriptsize{($\times \textbf{6.0}$)} \\ \bottomrule
     % [18.1 20.4 29.4] (scale=0.5), [17.2 28.  50.6] (scale=0.1), [16.9 23.6 37.3](scale=0.2), [18.  36.4 75.7](scale=0.05), [ 24.   67.7 187.2](scale=0.005)
    \end{tabular}
\end{table}


\begin{figure}
    \centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_992.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_323.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_985.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_130.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_89.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_604.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_900.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_779.jpeg}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\linewidth]{images/imagenet_guided_diff_progressive_hard_samples_class_0.jpeg}
    \end{subfigure}
    \caption{Progressive hardening of samples. TODO: Also display hardness score below each image.}
\end{figure}


\begin{figure}
    \centering
    \includegraphics{images/per_class_accuracy_baseline_synthetic.pdf}
    \caption{Top-1 per-class accuracy for synthetic data. We threshold the classes as the mean accuracy over real imagenet validation images, i.e., 77.6. Highlight ImageNet-400 in plot itself.}
\end{figure}



\begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet400_top1.pdf}
        \caption{ImageNet-400 (top-1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet400_top5.pdf}
        \caption{ImageNet-400 (top-5)}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet_top1.pdf}
        \caption{ImageNet (top-1)}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\linewidth]{images/comprehesive_eval_minimal_imagenet_top5.pdf}
        \caption{ImageNet (top-5)}
    \end{subfigure}
    \caption{Comprehensive evaluation of existing pre-trained models with increasing hardness score. To avoid statistical noise, we plot accuracy for each score range only when at least 5 images for each class are available. Given limited number of samples in real data, its not feasible to do a accurate evaluation of robustness over all score values. TODO: just for the sake of it, also provide full real-data curves in appendix.}
\end{figure}


\begin{table}[!htb]
    \centering
    \caption{Top-1 accuracy on original \textit{ImageNet-400} dataset and some of its domain shifted versions. (R) refers to using only real data where (R+S) refers to using real and synthetic data together in training. TODO: Also provide top-5 accuracy results.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc|cc} \toprule
        Architecture & Data & Original & ImageNet-Rendition & ImageNet-sketch  \\ \midrule
        \multirow{3}{*}{ResNet-18} & R & $88.4$ &  $28.9$ & $28.5$ \\
         & R + S (uniform) & $88.7$ \scriptsize{($\textbf{+0.3}$)} &  $29.5$ \scriptsize{($\textbf{+0.6}$)} & $31.1$ \scriptsize{($\textbf{+2.6}$)}  \\
         & R + S (\ours) & $88.3$ \scriptsize{($\textbf{-0.3}$)} &  $30.2$ \scriptsize{($\textbf{+1.3}$)} & $32.2$ \scriptsize{($\textbf{+3.7}$)} \\ \midrule
        \multirow{3}{*}{ResNet-50} & R & $91.6$ &  $32.5$ & $30.0$ \\
         & R + S (uniform) & $91.5$ \scriptsize{($\textbf{-0.1}$)} &  $33.4$ \scriptsize{($\textbf{+0.9}$)} & $34.3$ \scriptsize{($\textbf{+4.3}$)} \\
         & R + S (\ours) & $91.4$ \scriptsize{($\textbf{-0.2}$)} &  $33.9$ \scriptsize{($\textbf{+1.4}$)} & $35.4$ \scriptsize{($\textbf{+5.4}$)} \\ \midrule
        \multirow{3}{*}{ResNet-101} & Real & $92.4$ &  $34.7$ & $35.7$ \\
         & R + S (uniform) & $92.3$ \scriptsize{($\textbf{-0.1}$)} &  $36.1$ \scriptsize{($\textbf{+1.4}$)} & $38.7$ \scriptsize{($\textbf{+3.0}$)} \\
         & R + S (\ours) & $92.2$ \scriptsize{($\textbf{-0.2}$)} &  $36.2$ \scriptsize{($\textbf{+1.5}$)} & $38.6$ \scriptsize{($\textbf{+2.9}$)}  \\ \bottomrule
    \end{tabular}}
\end{table}

\begin{table}[!htb]
    \centering
    \caption{Top-1 accuracy on original full \textit{ImageNet-1K} dataset and some of its domain shifted versions. (R) refers to using only real data where (R+S) refers to using real and synthetic data together in training.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc|cc} \toprule
        Architecture & Data & Original & ImageNet-Rendition & ImageNet-sketch  \\ \midrule
        \multirow{3}{*}{ResNet-18} & R & $70.6$ &  $22.4$ & $23.0$ \\
         & R + S (uniform) & $70.2$ \scriptsize{($\textbf{-0.4}$)} &  $22.2$ \scriptsize{($\textbf{-0.2}$)} & $22.8$ \scriptsize{($\textbf{-0.2}$)}  \\
         & R + S (\ours) & $69.3$ \scriptsize{($\textbf{-1.3}$)} &  $22.2$ \scriptsize{($\textbf{-0.2}$)} & $22.6$ \scriptsize{($\textbf{-0.4}$)} \\ \midrule
        \multirow{3}{*}{ResNet-50} & R & $77.6$ &  $26.9$ & $27.4$ \\
         & R + S (uniform) & $77.2$ \scriptsize{($\textbf{-0.4}$)} &  $27.3$ \scriptsize{($\textbf{+0.4}$)} & $28.9$ \scriptsize{($\textbf{+1.5}$)} \\
         & R + S (\ours) & $77.1$ \scriptsize{($\textbf{-0.5}$)} &  $27.3$ \scriptsize{($\textbf{+0.4}$)} & $28.6$ \scriptsize{($\textbf{+1.2}$)} \\ \midrule
        \multirow{3}{*}{ResNet-101} & Real & $--$ &  $--$ & $--$ \\
         & R + S (\ours) & $--$ &  $--$ & $--$  \\ \bottomrule
    \end{tabular}}
\end{table}
